Decentralized Riemannian Algorithm for Nonconvex Minimax Problems

The minimax optimization over Riemannian manifolds (possibly nonconvex constraints) has been actively applied to solve many problems, such as robust dimensionality reduction and deep neural networks with orthogonal weights (Stiefel manifold). Although many optimization algorithms for minimax problems have been developed in the Euclidean setting, it is difficult to convert them into Riemannian cases, and algorithms for nonconvex minimax problems with nonconvex constraints are even rare. On the other hand, to address the big data challenges, decentralized (serverless) training techniques have recently been emerging since they can reduce communications overhead and avoid the bottleneck problem on the server node. Nonetheless, the algorithm for decentralized Riemannian minimax problems has not been studied. In this paper, we study the distributed nonconvex-strongly-concave minimax optimization problem over the Stiefel manifold and propose both deterministic and stochastic minimax methods. The Steifel manifold is a non-convex set. The global function is represented as the finite sum of local functions. For the deterministic setting, we propose DRGDA and prove that our deterministic method achieves a gradient complexity of $O( \epsilon^{-2})$ under mild conditions. For the stochastic setting, we propose DRSGDA and prove that our stochastic method achieves a gradient complexity of $O(\epsilon^{-4})$. The DRGDA and DRSGDA are the first algorithms for distributed minimax optimization with nonconvex constraints with exact convergence. Extensive experimental results on the Deep Neural Networks (DNNs) training over the Stiefel manifold demonstrate the efficiency of our algorithms.

==> proof.tex <==
\section{Experiments}
\subsection{Experimental Results of Distributionally Robust Optimization}
The experimental results of the distributionally robust optimization task are reported in Figures \ref{img:3} and \ref{img:4}.

\begin{figure*}[h]
\centering
\subfigure[MNIST]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/mnist_2_loss.png}
}
\subfigure[Fashion-MNIST]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/fmnist_2_loss.png}
}
\subfigure[CIFAR-10]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/cifar_2_loss.png}
}
% \vspace*{-6pt}
\caption{Training loss of different stochastic methods on the distributionally robust optimization task.}
\label{img:3}
% \vspace*{-6pt}
\end{figure*}

\begin{figure*}[h]
\centering
\subfigure[MNIST]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/mnist_2_acc.png}
}
\subfigure[Fashion-MNIST]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/fmnist_2_acc.png}
}
\subfigure[CIFAR-10]{
\hspace{0pt}
\includegraphics[width=.31\textwidth]{image/cifar_2_acc.png}
}
% \vspace*{-6pt}
\caption{Test accuracy of different methods on the distributionally robust optimization task.}
\label{img:4}
% \vspace*{-6pt}
\end{figure*}

\section{Theoretical Analysis}
\subsection{Consensus on the Stiefel Manifold}
In this subsection, we introduce some technical lemmas from previous works.

To solve the consensus problem over $\mathrm{St}(d,r)$ defined in \eqref{eq:12}, the Riemannian gradient method DRCS is proposed in \cite{chen2021local} as the following:  $\forall i \in [n]$,
% \begin{align} \label{eq:13}
% x_{i, k+1}=\mathcal{R}_{x_{i, k}}\left(\alpha \mathcal{P}_{\mathrm{T}_{x_{i}}\mathcal{M}}\left(\sum_{j=1}^{n} W_{i j}^{t} x_{j, k}\right)\right)
% \end{align}
\begin{align} \label{eq:13}
x_{i, t+1}=\mathcal{R}_{x_{i, t}}\left(\alpha \mathcal{P}_{\mathrm{T}_{x_{i,t}}\mathcal{M}}\left(\sum_{j=1}^{n} W_{i j}^{k} x_{j, t}\right)\right)
\end{align}

DRCS converges almost surely to consensus when $r \leq \frac{2}{3} d - 1$ with random initialization \cite{markdahl2020high}. Most importantly, DRCS has the local Q-linear convergence for decentralized optimization. Due to the nonconvexity of M, the Q-linear rate of DRCS holds in a local region defined as follows
% to study the decentralized optimization algorithm to solve (1.1), 
% is more important 

\begin{align} \label{eq:14}
\mathcal{N}: &=\mathcal{N}_{1} \cap \mathcal{N}_{2} \\
\mathcal{N}_{1} :&=\left\{\mathbf{x}:\|\mathbf{x}-\overline{\mathbf{x}}\|^{2} \leq n \delta_{1}^{2}\right\} \\
\mathcal{N}_{2}: &=\left\{\mathbf{x}:\|\mathbf{x}-\overline{\mathbf{x}}\|_{ \infty} \leq \delta_{2}\right\} 
\end{align}
where $\delta_{1}, \delta_{2}$ satisfy
\begin{align}
\delta_{1} & \leq \frac{1}{5 \sqrt{r}} \delta_{2} \quad \text { and } \quad \delta_{2} \leq \frac{1}{6}
\end{align}
In addition, we also need the following lemma:
\begin{lemma}  \citep{chen2021local} \label{lem:3}
(1) With doubly stochastic matrix $\mathbf{W}$, for some $\alpha 
\in (0,1]$, and $k \geq \lceil log_{\lambda_2} ( \frac{1}{2\sqrt{n}} ) \rceil$, the
sequence $\{x_t\}$ from \eqref{eq:13} achieves consensus linearly if the initialization satisfies $x_0 \in \mathcal{N}$. That is, there exists $\rho_k \in $(0,1) such that $x_t \in \mathcal{N}$ for all $t \geq 0$ and
\begin{align}
\|x_{t+1} - \hat{x}_{t+1}\| \leq \rho_k \| x_t - \hat{x}_t \|    
\end{align}
(2) Denote the smallest eigenvalue of  $\mathbf{W}^k$ by $\lambda_n (\mathbf{W}^k)$, and the Lipschitz constant $L_k = 1 - \lambda_n (\mathbf{W}^k)$, it follows that
\begin{align}
\left\|\sum_{i=1}^{n} \mathrm{grad} J^{k}\left(x_{i}\right)\right\| \leq L_{k}\|\mathbf{x}-\hat{\mathbf{x}}\|^{2}   
\end{align}
and  
\begin{align}
\left\|\mathrm{grad} J^{k}(\mathbf{x})\right\| \leq L_{k} \|\mathbf{x} - \hat{\mathbf{x}}\|
\end{align}
We could know $L_k \in (0, 2]$ and we could choose $L_k$ as 2.
% Moreover, suppose $\mathbf{x} \in \mathcal{N}_{2}$. We then have
% \begin{align}
% \max _{i \in[n]}\left\|\mathrm{grad} J_{i}^{k}(\mathbf{x})\right\| \leq 2 \delta_{2} .    
% \end{align} 

(3) For any $\mathbf{x} \in \mathrm{St}(d, r)^{n}$, we have
\begin{align}
\|\bar{x}-\hat{x}\| \leq \frac{2 \sqrt{r}\|\mathbf{x}-\hat{\mathbf{x}}\|^{2}}{n}
\end{align}
and suppose $\mathbf{x}_1, \mathbf{x}_2 \in \mathcal{N}_{1}$,
% And $\hat{x}_1$ and $\hat{x}_2$ are the IAM of $x_1^{1}, \ldots, x_1^{n}$ and $x_{2}^{1}, \ldots, x_{2}^{n}$, respectively. 
then we have 
\begin{align}
\|\hat{x}_1 - \hat{x}_2\| \leq \frac{1}{1-2 \delta_{1}^{2}}\|\bar{x}_1 - \bar{x}_2\|,
\end{align}
\end{lemma}

% \begin{lemma} \citep{chen2021local} \label{lem:5}
% For any $\mathbf{x} \in \mathrm{St}(d, r)^{n}$, let $\bar{x} = \frac{1}{n} \sum_{i=1}^{n} x_{i}$ be the Euclidean mean and denote $\bar{\mathbf{x}}=\mathbf{1}_{n} \otimes \bar{x}$. Similarly, let $\hat{x}$ is the IAM and  $\hat{\mathbf{x}}=\mathbf{1}_{n} \otimes \hat{x}$,. Moreover, if $\|\mathbf{x}- \bar{\mathbf{x}}\|^{2} \leq n / 2$, one has
% \begin{align}
% \|\bar{x}-\hat{x}\| \leq \frac{2 \sqrt{r}\|\mathbf{x}-\hat{\mathbf{x}}\|^{2}}{n}
% \end{align}
% \end{lemma}
% Then we use following lemma to bound the Euclidean distance between two average points $\hat{x}_{t}$ and $\hat{x}_{t+1}$.
% \begin{lemma} \citep{chen2021local} \label{lem:6}
% Suppose $\mathbf{x}_1, \mathbf{x}_2 \in \mathcal{N}_{1}$. And $\hat{x}_1$ and $\hat{x}_2$ are the IAM of $x_1^{1}, \ldots, x_1^{n}$ and $x_{2}^{1}, \ldots, x_{2}^{n}$, respectively. Then we have 
% \begin{align}
% \|\hat{x}_1 - \hat{x}_2\| \leq \frac{1}{1-2 \delta_{1}^{2}}\|\bar{x}_1 - \bar{x}_2\|,
% \end{align}
% \end{lemma}

\subsection{Basic Lemma}
Subsequently, we move on to the update of variable y.

\begin{lemma}  (Restatement of Lemma 2) 
% Under the assumptions, 
The gradient of function $\Phi(x) = \max_{y\in \mathcal{Y}} F(x, y)$ is $L_{\Phi}$-Lipschitz,
% with respect to retraction
and the function $y^{*}(x) = \arg \max_{y \in \mathcal{Y}} \Phi(x, y) $ is $\kappa$-Lipschitz.
% with respect to retraction. 
Specifically, $\forall x_1, x_2 \in \mathcal{M} $ 
% and $u \in \mathcal{T}_{x_1} \mathcal{M}$, 
we have
\begin{align}
\|y^{*}(x_1) - y^{*}(x_2) \| &\leq \kappa \|x_1 - x_2\| \nonumber\\
\| \mathrm{grad}\Phi(x_1) - \mathrm{grad}\Phi(x_2) \| &\leq L_{\Phi} \|x_1 - x_2\|  \nonumber
\end{align}
where 
$L_{\Phi} = \kappa L_{12} + L_{11}$,and $\kappa = L_{21} / \mu$ denotes the number condition.
\begin{proof}
Given any $x_{1}, x_{2}
% =R_{x_{1}}(u) 
\in \mathcal{M}$ 
% and $u \in T_{x_{1}} \mathcal{M}$
, define $y^{*}\left(x_{1}\right)=\arg \max _{y \in \mathcal{Y}} F\left(x_{1}, y\right)$ and $y^{*}\left(x_{2}\right)=$ $\arg \max _{y \in \mathcal{Y}} F\left(x_{2}, y\right)$. Under the Assumption \ref{ass:2}, 
% the function $F\left(x_{1}, \cdot\right)$ is $\mu$-strongly concave, 
we have
\begin{align}
&F\left(x_{1}, y^{*}\left(x_{1}\right)\right) \leq F\left(x_{1}, y^{*}\left(x_{2}\right)\right)+\left(\nabla_{y} F\left(x_{1}, y^{*}\left(x_{2}\right)\right)\right)^{T}\left(y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right)-\frac{\mu}{2}\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\|^{2}  \label{eq:32}\\
&F\left(x_{1}, y^{*}\left(x_{2}\right)\right) \leq F\left(x_{1}, y^{*}\left(x_{1}\right)\right)+\left(\nabla_{y} F\left(x_{1}, y^{*}\left(x_{1}\right)\right)\right)^{T}\left(y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right)-\frac{\mu}{2}\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\|^{2}  \label{eq:33}
\end{align}
Based on  the inequalities \eqref{eq:32} and  \eqref{eq:33}, we obtain
\begin{align} \label{eq:34}
\left(y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right)^{T}\left(\nabla_{y} F\left(x_{1}, y^{*}\left(x_{2}\right)\right)-\nabla_{y} F\left(x_{1}, y^{*}\left(x_{1}\right)\right)\right)+\mu\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\|^{2} \leq 0 .
\end{align}
In addition, since $\mathcal{Y}$ is a convex set, we have
\begin{align}
\left(y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right)^{T} \nabla_{y} F\left(x_{1}, y^{*}\left(x_{1}\right)\right) \leq 0 \label{eq:35}\\
\left(y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right)^{T} \nabla_{y} F\left(x_{2}, y^{*}\left(x_{2}\right)\right) \leq 0 \label{eq:36}
\end{align}
By combining above two inequalities, we have
\begin{align} \label{eq:37}
\left(y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right)^{T}\left(\nabla_{y} F\left(x_{1}, y^{*}\left(x_{1}\right)\right)-\nabla_{y} F\left(x_{2}, y^{*}\left(x_{2}\right)\right)\right) \leq 0 .    
\end{align}
By plugging the inequalities \eqref{eq:37} into \eqref{eq:34}, we have
\begin{align}
\mu\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\|^{2} & \leq\left(y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right)^{T}\left(\nabla_{y} F\left(x_{2}, y^{*}\left(x_{2}\right)\right)-\nabla_{y} F\left(x_{1}, y^{*}\left(x_{2}\right)\right)\right) \nonumber\\
& \leq\left\|y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right\|\left\|\nabla_{y} F\left(x_{2}, y^{*}\left(x_{2}\right)\right)-\nabla_{y} F\left(x_{1}, y^{*}\left(x_{2}\right)\right)\right\| \nonumber\\
& \leq L_{21}\|x_1 - x_2\|\left\|y^{*}\left(x_{2}\right)-y^{*}\left(x_{1}\right)\right\|
\end{align}
Thus, we have
\begin{align}
\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\| \leq L_{21} / \mu\|x_1 - x_2\|,
\end{align}
For the second inequality in the Lemma \ref{lem:3}, we have 
\begin{align}
&\left\|\mathrm{grad} \Phi\left(x_{1}\right) - \mathrm{grad} \Phi\left(x_{2}\right)\right\| \nonumber\\
=&\left\|\mathrm{grad}_{x} F\left(x_{1}, y^{*}\left(x_{1}\right)\right)- \mathrm{grad}_{x} F\left(x_{2}, y^{*}\left(x_{2}\right)\right)\right\| \nonumber\\
\leq& \left\|\mathrm{grad}_{x} F\left(x_{1}, y^{*}\left(x_{1}\right)\right) - \mathrm{grad}_{x} F\left(x_{1}, y^{*}\left(x_{2}\right)\right)\right\| + \left\|\mathrm{grad}_{x} F\left(x_{1}, y^{*}\left(x_{2}\right)\right) -  \mathrm{grad}_{x} F\left(x_{2}, y^{*}\left(x_{2}\right)\right)\right\| \nonumber\\
\leq& L_{12}\left\|y^{*}\left(x_{1}\right)-y^{*}\left(x_{2}\right)\right\|+L_{11}\|x_2 - x_1\| \nonumber\\
\leq& \left(\kappa L_{12}+L_{11}\right)\|x_2 - x_1\|
\end{align}
\end{proof}
\end{lemma} 

 
\begin{lemma} \label{lem:5}
Under the above assumptions, and set $0 < \eta   \leq 1$ and $0 < \lambda \leq 1$, for the Algorithm \ref{alg:1}, we have
\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2}-\frac{3 \eta^2}{4}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+\frac{25 \eta}{6 \mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
For the Algorithm \ref{alg:2}, we have
\begin{align}
\mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \mathbb{E}\left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\mathbb{E}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2}-\frac{3 \eta^2}{4}\mathbb{E}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+\frac{25 \eta}{6 \mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\mathbb{E}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
where $\kappa=L_{21} / \mu$ and $L =\max \left(1, L_{11}, L_{12}, L_{21}, L_{22}\right)$.

\begin{proof}

$\textbf{P.1. Proof for algorithm \ref{alg:1}}$

The function $F(x, y)$ is $L$-smooth w.r.t $y$, we have
\begin{align}
F\left(\hat{x}_{t}, \bar{y}_{t+1}\right) -  F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right), \bar{y}_{t+1} -  \bar{y}_{t}\right\rangle   \geq - \frac{L}{2}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} 
\end{align}
Since the function $F(x, y)$ is $\mu$-strongly concave w.r.t $y$, we also have
\begin{align}
F\left(\hat{x}_{t}, y^{*}(\bar{x}_{t})\right) \leq & F\left(\hat{x}_{t}, \bar{y}_{t}\right)+\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right), y^{*}(\bar{x}_{t}) - \bar{y}_{t}\right\rangle-\frac{\mu}{2}\left\|y^{*}(\bar{x}_{t}) - \bar{y}_{t}\right\|^{2} \nonumber\\
=& F\left(\hat{x}_{t}, \bar{y}_{t}\right) + \left\langle \bar{v}_{t}, y^{*}(\bar{x}_{t}) - \bar{y}_{t+1}\right\rangle+\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}, y^{*}(\bar{x}_{t}) - \bar{y}_{t+1}\right\rangle \nonumber\\
& + \left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right), \bar{y}_{t+1} - \bar{y}_{t}\right\rangle - \frac{\mu}{2}\left\|y^{*}(\bar{x}_{t})-\bar{y}_{t}\right\|^{2} .
\end{align}

Combining above two inequalities, we obtain
\begin{align} \label{eq:43}
0 \leq  \left\langle \bar{v}_{t}, y^{*}(\bar{x}_{t}) - \bar{y}_{t+1}\right\rangle + \left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}, y^{*}(\bar{x}_{t}) - \bar{y}_{t+1}\right\rangle  - \frac{\mu}{2}\left\|y^{*}(\bar{x}_{t}) - \bar{y}_{t}\right\|^{2} + \frac{L}{2}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2}
\end{align}
where we also use the fact that $F\left(\hat{x}_{t}, y^{*}(\bar{x}_{t})\right) \geq F\left(\hat{x}_{t}, \bar{y}_{t + 1}\right)$. According to the update step of $y$, we have
\begin{align} \label{eq:44}
\left\langle \bar{v}_{t}, y^{*}(\bar{x}_{t})  - \bar{y}_{t+1}\right\rangle & \leq \frac{1}{\eta}\left\langle \bar{y}_{t+1} - \bar{y}_{t}, y^{*}(\bar{x}_{t})  - \bar{y}_{t+1} \right\rangle \nonumber\\
&=-\frac{1}{\eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2}+\frac{1}{\eta}\left\langle\bar{y}_{t+1} - \bar{y}_{t}, y^{*}(\bar{x}_{t}) -  \bar{y}_{t}\right\rangle
\end{align}
Putting the inequality \eqref{eq:44} into  \eqref{eq:43}, we have
\begin{align} \label{eq:45}
0 \leq & \left\langle  \bar{v}_{t}, y^{*}(\hat{x}_{t}) - \bar{y}_{t}\right\rangle + \left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}, y - \bar{y}_{t+1}\right\rangle \nonumber\\
& - \frac{1}{\eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} - \frac{\mu}{2}\left\|y^{*}(\bar{x}_{t}) - \bar{y}_{t}\right\|^{2} + \frac{L}{2}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2}
\end{align}
As  we have
\begin{align}
 \left\langle \bar{v}_{t}, y^{*}\left(\hat{x}_{t}\right) - y_{t}\right\rangle \leq \frac{1}{2 \eta} \left\|\bar{y}_{t} - y^{*}\left(\bar{x}_{t}\right)\right\|^{2} + \frac{1}{2 \eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} - \frac{1}{2 \eta}\left\|\bar{y}_{t+1} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2}
\end{align}
And by Cauchy-Schwartz inequality we also have
\begin{align}
&\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) -\bar{v}_{t}, y^{*}\left(\bar{x}_{t}\right) - \bar{y}_{t+1}\right\rangle \nonumber\\
&=\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}, y^{*}\left(\hat{x}_{t}\right) - \bar{y}_{t}\right\rangle + \left\langle\nabla_{y} F\left(x_{t}, y_{t}\right) - \bar{v}_{t}, \bar{y}_{t} - \bar{y}_{t+1}\right\rangle \nonumber\\
&\leq \frac{1}{\mu}\left\|\nabla_{y} F\left(\bar{x}_{t}, \bar{y}_{t}\right) - \bar{w}_{t}\right\|^{2} + \frac{\mu}{4}\left\|y^{*}\left(\hat{x}_{t}\right) - \bar{y}_{t}\right\|^{2} + \frac{1}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{\mu}{4}\left\|\bar{y}_{t} - \bar{y}_{t+1}\right\|^{2} \nonumber\\
&=\frac{2}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{\mu}{4}\left\|y^{*}\left(\hat{x}_{t}\right) - \bar{y}_{t}\right\|^{2} + \frac{\mu}{4}\left\|\bar{y}_{t}-\bar{y}_{t+1}\right\|^{2}
\end{align}

Then \eqref{eq:45} is equivalent to
\begin{align}
\frac{1}{2 \eta}\left\|\bar{y}_{t+1} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &\left(\frac{1}{2 \eta} - \frac{\mu}{4}\right)\left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} + \left(\frac{1}{2 \eta} + \frac{\mu}{4} + \frac{L}{2}-\frac{1}{\eta}\right)\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} \nonumber\\
&+\frac{2}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} \nonumber\\
\leq &\left(\frac{1}{2 \eta} - \frac{\mu}{4}\right)\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} + \left(\frac{3 L}{4}-\frac{1}{2 \eta}\right)\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} + \frac{2}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} \nonumber\\
% =&\left(\frac{1}{2 \eta} - \frac{\mu}{4}\right)\left\|\bar{y}_{t} - y^{*}\left(\bar{x}_{t}\right)\right\|^{2} - \left(\frac{3}{8 \eta} + \frac{1}{8 \eta}-\frac{3 L}{4}\right)\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} \nonumber\\
% &+\frac{2}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} \nonumber\\
\leq &\left(\frac{1}{2 \eta}-\frac{\mu}{4}\right)\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \frac{3}{8 \eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} + \frac{2}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2}
\end{align}
where the second inequality holds by $L \geq \mu$ and $0<\eta \leq 1$, and the last inequality is due to $0<\eta \leq \frac{1}{6 L}$. It can be reformulated as
\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq\left(1 - \frac{\eta \mu}{2}\right)\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \frac{3}{4}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} + \frac{4 \eta}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2}
\end{align}
According to Young’s inequality we have:
\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} 
& \leq\left(1+\frac{\eta \mu}{4}\right)\left\|\bar{y}_{t+1}-y^{*}\left(x_{t}\right)\right\|^{2}+\left(1+\frac{4}{\eta \mu}\right)\left\|y^{*}\left(\hat{x}_{t}\right)-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} \nonumber\\
& \leq\left(1+\frac{\eta \mu}{4}\right)\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2}+\left(1+\frac{4}{\eta \mu}\right)  \kappa^{2}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}

where the first inequality holds by the Cauchy-Schwarz inequality and Young's inequality, and the last equality is due to Lemma \ref{lem:2}.
By combining the above inequalities, we have

\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} \leq &\left(1+\frac{\eta \mu}{4}\right)\left(1-\frac{\eta \mu}{2}\right)\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \left(1+\frac{\eta \mu}{4}\right) \frac{3 \eta^2}{4}\left\| \bar{v}_{t}\right\|^{2} \nonumber\\
& + \left(1+\frac{\eta \mu }{4}\right) \frac{4 \eta}{\mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{w}_{t}\right\|^{2} + \left(1+\frac{4}{\eta \mu}\right) \kappa^{2}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
Since $0 < \eta \leq \frac{1}{6 L}$ and $ L \geq \mu$, we have 
% $\lambda \leq \frac{1}{6 \tilde{L}} \leq \frac{1}{6 \mu}$ and $\eta_{t} \leq 1 \leq \frac{1}{6 \mu \lambda}$. Then we obtain
\begin{align}
\left(1+\frac{\eta \mu}{4}\right)\left(1 - \frac{\eta \mu }{2}\right) &= 1 - \frac{\eta \mu}{2} + \frac{\eta \mu}{4} - \frac{\eta^{2} \mu^{2} }{8} \leq 1 - \frac{\eta \mu}{4} \\
- \left(1+\frac{\eta \mu}{4}\right) \frac{3 \eta^2}{4} & \leq - \frac{3 \eta^2}{4} \\
\left(1 + \frac{\eta \mu}{4}\right) \frac{4 \eta}{\mu} & \leq \left(1 + \frac{1}{24}\right) \frac{4 \eta}{\mu}=\frac{25 \eta}{6 \mu} 
% \\\left(1 + \frac{4}{\eta \mu}\right) \kappa^{2} \eta^{2} &= \gamma^{2} \kappa^{2} \eta_{t}^{2} + \frac{4 \gamma^{2} \kappa^{2} \eta_{t}}{\mu \lambda} \leq \frac{ \kappa^{2} \eta_{t}}{6 \mu \lambda}+\frac{4  \kappa^{2} \eta_{t}}{\mu \lambda}=\frac{25  \kappa^{2} \eta}{6 \mu}
\end{align}

Finally, we have 
\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2}-\frac{3 \eta^2}{4}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+\frac{25 \eta}{6 \mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
$\textbf{P.2. Proof for algorithm \ref{alg:2}}$
Similarly, we have \eqref{eq:45} as following: 
\begin{align} 
0 \leq & \left\langle  \bar{\underline{v}}_{t}, y^{*}(\hat{x}_{t}) - \bar{y}_{t}\right\rangle + \left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{\underline{v}}_{t}, y - \bar{y}_{t+1}\right\rangle \nonumber\\
& - \frac{1}{\eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} - \frac{\mu}{2}\left\|y^{*}(\bar{x}_{t}) - \bar{y}_{t}\right\|^{2} + \frac{L}{2}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2}
\end{align}
As  we have
\begin{align}
 \left\langle \bar{\underline{v}}_{t}, y^{*}\left(\hat{x}_{t}\right) - y_{t}\right\rangle \leq \frac{1}{2 \eta} \left\|\bar{y}_{t} - y^{*}\left(\bar{x}_{t}\right)\right\|^{2} + \frac{1}{2 \eta}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} - \frac{1}{2 \eta}\left\|\bar{y}_{t+1} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2}
\end{align}
Similarly, taking expectation on both side, we have 
\begin{align}
&\mathbb{E}[\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) -\bar{\underline{v}}_{t}, y^{*}\left(\bar{x}_{t}\right) - \bar{y}_{t+1}\right\rangle] \nonumber\\
=&\mathbb{E}[\left\langle\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}, y^{*}\left(\hat{x}_{t}\right) - \bar{y}_{t}\right\rangle] + \mathbb{E}[ \left\langle\nabla_{y} F\left(x_{t}, y_{t}\right) - \bar{v}_{t}, \bar{y}_{t} - \bar{y}_{t+1}\right\rangle] \nonumber\\
=&\frac{2}{\mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{\mu}{4}\mathbb{E}\left\|y^{*}\left(\hat{x}_{t}\right) - \bar{y}_{t}\right\|^{2} + \frac{\mu}{4}\mathbb{E}\left\|\bar{y}_{t}-\bar{y}_{t+1}\right\|^{2}
\end{align}

Then we have 
\begin{align}
\mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq \left(1 - \frac{\eta \mu}{2}\right)\mathbb{E}\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \frac{3}{4}\mathbb{E}\left\|\bar{y}_{t+1} - \bar{y}_{t}\right\|^{2} + \frac{4 \eta}{\mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2}
\end{align}
Then 
\begin{align}
\mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} \leq &\left(1+\frac{\eta \mu}{4}\right)\left(1-\frac{\eta \mu}{2}\right)\mathbb{E}\left\|\bar{y}_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \left(1+\frac{\eta \mu}{4}\right) \frac{3 \eta^2}{4}\mathbb{E}\left\| \bar{\underline{v}}_{t}\right\|^{2} \nonumber\\
& + \left(1+\frac{\eta \mu }{4}\right) \frac{4 \eta}{\mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \left(1+\frac{4}{\eta \mu}\right) \kappa^{2}\mathbb{E}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
Finally, we have 
\begin{align}
\mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \mathbb{E}\left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\mathbb{E}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2}-\frac{3 \eta^2}{4}\mathbb{E}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+\frac{25 \eta}{6 \mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\mathbb{E}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}



\end{proof}
\end{lemma}

\begin{lemma} \label{lem:6}
For algorithm \ref{alg:1}:
\begin{align} 
&\left\|\mathbf{y}_{t} -  \bar{\mathbf{y}}_{t}\right\|^{2} \leq\left(1 + c_{0}\right) \lambda^{2}\left\|\mathbf{y}_{t-1} -  \bar{\mathbf{y}}_{t-1}\right\|^{2} + \left(1 + \frac{1}{c_{0}}\right) \eta^{2}\left\|\mathbf{v}_{t-1} -  \bar{\mathbf{v}}_{t-1}\right\|^{2} \label{eq:64}\\
&\left\|\mathbf{v}_{t} - \bar{\mathbf{v}}_{t}\right\|^{2} \leq \left(1 + c_{0}\right) \lambda^{2} \left\|\mathbf{v}_{t-1} - \bar{\mathbf{v}}_{t-1}\right\|^{2} + \left(1 + \frac{1}{c_{0}}\right)\left\|\nabla_y F(x_t, y_t) - \nabla_y F(x_{t-1}, y_{t-1})\right\|^{2} \label{eq:65}\\
&\left\|\mathbf{y}_{t}-\mathbf{y}_{t-1}\right\|^{2} \leq 8\left\|\left(\mathbf{y}_{t-1} -  \bar{\mathbf{y}}_{t-1}\right)\right\|^{2} + 4 \eta^{2}\left\|\mathbf{v}_{t-1} - \bar{\mathbf{v}}_{t-1}\right\|^{2} + 4 \eta^{2} n\left\|\bar{v}_{t-1}\right\|^{2} \label{eq:66}
\end{align}
Similarly, For algorithm \ref{alg:2}, we have \begin{align}
&\left\|\mathbf{y}_{t} -  \bar{\mathbf{y}}_{t}\right\|^{2} \leq\left(1 + c_{0}\right) \lambda^{2}\left\|\mathbf{y}_{t-1} -  \bar{\mathbf{y}}_{t-1}\right\|^{2} + \left(1 + \frac{1}{c_{0}}\right) \eta^{2}\left\|\mathbf{\underline{v}}_{t-1} -  \bar{\mathbf{\underline{v}}}_{t-1}\right\|^{2} \label{eq:67}\\
&\left\|\mathbf{\underline{v}}_{t} - \bar{\mathbf{\underline{v}}}_{t}\right\|^{2} \leq \left(1 + c_{0}\right) \lambda^{2} \left\|\mathbf{\underline{v}}_{t-1} - \bar{\mathbf{\underline{v}}}_{t-1}\right\|^{2} + \left(1 + \frac{1}{c_{0}}\right)\left\|\nabla_y F(x_t, y_t; \mathcal{B}_{t}) - \nabla_y F(x_{t-1}, y_{t-1}; \mathcal{B}_{t-1})\right\|^{2} \label{eq:68}\\
&\left\|\mathbf{y}_{t}-\mathbf{y}_{t-1}\right\|^{2} \leq 8\left\|\left(\mathbf{y}_{t-1} -  \bar{\mathbf{y}}_{t-1}\right)\right\|^{2} + 4 \eta^{2}\left\|\mathbf{\underline{v}}_{t-1} - \bar{\mathbf{\underline{v}}}_{t-1}\right\|^{2} + 4 \eta^{2} n\left\|\bar{\underline{v}}_{t-1}\right\|^{2} \label{eq:69}
\end{align}

\begin{proof}
We firstly consider the \eqref{eq:64}
\begin{align}
\left\|\mathbf{y}_{t} - \mathbf{\bar{y}}_{t}\right\|^{2} =& \left\|\mathbf{W} \mathbf{y}_{t} - \eta  \mathbf{v}_{t-1} - \mathbf{1} \otimes \left(\bar{y}_{t-1} - \eta \bar{v}_{t-1}\right)\right\|^{2} \nonumber\\ 
\leq& \left(1 + c_{0}\right)\left\|\mathbf{W}   \mathbf{y}_{t-1} - \mathbf{1} \otimes \bar{v}_{t-1}\right\|^{2} + \left(1+\frac{1}{c_{0}}\right) \eta^{2}\left\|\mathbf{v}_{t-1} - \mathbf{1} \otimes \bar{v}_{t-1}\right\|^{2} \nonumber\\
\leq& \left(1+c_{0}\right) \lambda^{2}\left\|\mathbf{y}_{t-1} - \mathbf{1} \otimes \overline{y}_{t-1}\right\|^{2} + \left(1+\frac{1}{c_{0}}\right) \eta^{2}\left\|\mathbf{v}_{t-1} - \mathbf{1} \otimes \bar{v}_{t-1}\right\|^{2}.
\end{align}
Subsequently, we consider the proof of \eqref{eq:66}
\begin{align}
\left\|\mathbf{y}_{t} - \mathbf{y}_{t-1}\right\|^{2} 
=& \left\|(\mathbf{W} - \mathbf{I}) \mathbf{y}_{t-1} - \eta \mathbf{v}_{t-1}\right\|^{2} \nonumber\\
\leq& 2\left\|(\mathbf{W} - \mathbf{I}) \mathbf{y}_{t-1}\right\|^{2}+2 \eta^{2}\left\|\mathbf{v}_{t-1}\right\|^{2} \nonumber\\
=& 2\left\|(\mathbf{W} - \mathbf{I})\left(\mathbf{y}_{t-1} - \mathbf{1} \otimes \bar{\mathbf{y}}_{t-1}\right)\right\|^{2} + 2 \eta^{2}\left\|\mathbf{v}_{t-1}\right\|^{2} \nonumber\\
\leq & 8\left\|\left(\mathbf{y}_{t-1} - \mathbf{1} \otimes \bar{y}_{t-1}\right)\right\|^{2}+4 \eta^{2}\left\|\mathbf{v}_{t-1}-\mathbf{1} \otimes \bar{\mathbf{v}}_{t-1}\right\|^{2}+4 \eta^{2} n\left\|\bar{\mathbf{v}}_{t-1}\right\|^{2}
\end{align}
Similarly, we get the inequalities \eqref{eq:65}, \eqref{eq:67}, and \eqref{eq:68}, and \eqref{eq:69}.
\end{proof}
\end{lemma}
\begin{lemma} \citep{xu2015augmented} \label{lem:7}
Let $\left\{V_{t}\right\}_{t \geq 0}$ and $\left\{C_{t}\right\}_{t \geq 0}$  be non-negative sequences.
\vspace*{-6pt}
$$
U_{t+1} \leq a U_{t} + V_{t},
$$
where $0 < a < 1$. Then we have
$$
\sum_{i=0}^{t} U_{i}^{2} \leq \frac{2}{(1 - a)^{2}} \sum_{i=0}^{t} V_{i}^{2} + \frac{2}{1 - a^{2}} U_{0}^{2},
$$
\end{lemma}

\subsection{Convergence Analysis of DRGDA Algorithms}

\begin{lemma} \label{lem:8}
If $\mathbf{x}_{t} \in \mathcal{N}, \mathbf{x}_{t+1} \in \mathcal{N}_{1}$ and $x_{t+1}^i = \mathcal{R}_{x_{t}^i}\left(-\alpha \mathrm{grad} J{i}^{k}\left(\mathbf{x}_{t}\right) + \beta w_{t}^i\right)$, where $w_{t}^i \in \mathrm{T}_{x_{t}^i} \mathcal{M}$, $0 \leq \alpha \leq \frac{1}{M}, \beta \geq 0$. It follows that
\begin{align}
\left\|\hat{x}_{t}-\hat{x}_{t+1}\right\| \leq \frac{1}{1-2 \delta_{1}^{2}}\left(\frac{2 L_{t}^{2} \alpha + L_{t} \alpha}{n} \left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\beta\left\|\bar{w}_{t}\right\| + \frac{2 M \beta^{2}}{n}\left\|\mathbf{w}_{k}\right\|^{2}\right)
\end{align}
\begin{proof}
\vspace*{-6pt}
\begin{align}
\vspace*{-6pt}
&\left\|\bar{x}_{t+1} - \bar{x}_{t}\right\|
\leq \|\bar{x}_{t} + \frac{1}{n} \sum_{i=1}^{n}\left(-\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) + \beta w_{t}^i\right) - \bar{x}_{t+1}\| + \|\frac{1}{n} \sum_{i=1}^{n}\left(-\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) + \beta w_{t}^i\right)\| \nonumber\\
\leq & \frac{M}{n} \sum_{i=1}^{n}\left\|\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) + \beta w_{i, t}\right\|^{2}+\alpha\left\|\frac{1}{n} \sum_{i=1}^{n} \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right)\right\| + \beta\left\|\bar{w}_{t}\right\| \nonumber\\
\leq & \frac{2 M \alpha^{2}}{n}\left\|\mathrm{grad} J^{k} \left(\mathbf{x}_{t}\right)\right\|^{2} + \frac{2 M \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \alpha\left\|\frac{1}{n} \sum_{i=1}^{n} \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right)\right\| + \beta\left\|\bar{w}_{t}\right\| \nonumber\\
\leq & \frac{2 L_{t}^{2} M \alpha^{2} + L_{t} \alpha}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\frac{2 M \beta^{2}}{n}\left\|\mathbf{w}_{t}\right\|^{2} + \beta\left\|\bar{w}_{t}\right\| 
\end{align}
where the second inequality holds by Lemma \ref{lem:1} and the last inequality holds by Lemma \ref{lem:3} (2).

Therefore, based on Lemma \ref{lem:3} (3), we have 
\begin{align}
\left\|\hat{x}_{k}-\hat{x}_{k+1}\right\| \leq \frac{1}{1-2 \delta_{1}^{2}}\left\|\bar{x}_{k}-\bar{x}_{k+1}\right\| \leq \frac{1}{1-2 \delta_{1}^{2}}\left(\frac{2 L_{t}^{2} \alpha+L_{t} \alpha}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \beta\left\|\bar{w}_{t}\right\| + \frac{2 M \beta^{2}}{n}\left\|\mathbf{w}_{t}\right\|^{2}\right),
\end{align}
where we use the fact that $\alpha \leq \frac{1}{M}$.
\end{proof}
\end{lemma}

\begin{lemma} \label{lem:9}
Under assumptions \ref{ass:1}, and let $x_t \in \mathcal{N}$, $k \geq \lceil log_{\lambda_2} ( \frac{1}{2\sqrt{n}} ) \rceil$, then $\|v_t^i \| \leq 5D \forall i \in [n]$. If $x_t \in N$ and $\forall t \geq 0$. And following holds:
\begin{align} \label{eq:77}
\frac{1}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq 25C_{1}D^2 \beta^{2}, k \geq 0 .
\end{align}

\begin{proof}
Firstly, let $\bar{g}_{-1}=\bar{u}_0$. Basd on assumption, we have  
\begin{align}
\left\|u_{0}^i - \bar{g}_{-1}\right\| \leq\left\|u_{0}^i\right\|+\left\|\bar{g}_{-1}\right\| \leq 2 D
\end{align}
\end{proof}
\end{lemma}
% Since $\left\|w_{i, k}\right\| = \left\|\mathcal{P}_{T_{x_t^i \mathcal{M}}} u_{t}^i\right\| \leq\left\|u_{t}^i\right\|$. 
% Following the same argument in the proof of Lemma 4.1, we get $\mathbf{x}_{k+1} \in \mathcal{N}$ since $0<\alpha \leq \min \left\{\frac{\Phi}{2 L_{t}}, 1, \frac{1}{M}\right\}$ and $0 \leq \beta \leq \min \left\{\frac{1-\rho_{t}}{L_{G}+2 D} \delta_{1}, \frac{\alpha \delta_{1}}{5\left(L_{G}+2 D\right)}\right\}$
Following the Lemma4.1 \cite{chen2021decentralized}, we get $x_{t+1} \in N$ since $0 < \alpha \leq \bar{\alpha}$ where $ \bar{\alpha} = \min \left\{\frac{1}{2 L_{t}}, 1, \frac{1}{M}\right\}$ and $0 \leq \beta \leq \bar{\beta} $ where $\bar{\beta} =  \min \left\{\frac{1 - \rho_{k}}{5D} \delta_{1}, \frac{\alpha \delta_{1}}{10 D}\right\}$. 
Then, we have
\begin{align}
\left\|u_{t+1}^i - \bar{g}_{t}\right\| &=\left\|\sum_{j=1}^{n} W_{i, j}^{k} u_{t}^j - \bar{g}_{t} + \mathrm{grad}_x f\left(x_{ t+1}^i, y_{t+1}^i\right) - \mathrm{grad}_x f\left(x_{t}^i, y_t^i\right)\right\|  \nonumber\\
&=\left\|\sum_{j=1}^{n}\left(W_{i, j}^{t}-\frac{1}{n}\right)\left(u_{t}^j - \bar{g}_{t-1}\right) + \mathrm{grad}_x f\left(x_{ t+1}^i, y_{t+1}^i\right) - \mathrm{grad}_x f\left(x_{t}^i, y_t^i\right)\right\| \nonumber\\
& \leq \sigma_{2}^{t} \sqrt{n}\left\|u_{t}^j - \bar{g}_{t-1}\right\| + 2D  \nonumber\\
& \leq \frac{1}{2}\left\|u_t^i - \bar{g}_{k-1}\right\| + 2 D  \nonumber\\
& \leq 4D 
\end{align}

Hence, $\left\|u_{t+1}^i\right\| \leq \left\|u_{i, t+1} - \bar{g}_{t}\right\| + \left\|\bar{g}_{t}\right\| \leq 5 D$, where we use $\left\|\hat{g}_{t}\right\| \leq D$. 

Using the same argument of Lemma4.1 \cite{chen2021decentralized}, there exists some $C_{1}=\mathcal{O}\left(\frac{1}{\left(1-\rho_{t}\right)^{2}}\right)$ that is independent of $L$ and $D$ such that
\begin{align} \label{eq:77}
\frac{1}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq 25C_{1}D^2 \beta^{2}, k \geq 0 .
\end{align}

\begin{lemma} \label{lem:10} If we define 
\begin{align}
\mathbf{g}_{t}:=\left[\begin{array}{c}
\mathrm{grad}_x f_{1}\left(x_{t}^1, y_{t}^1\right) \\
\vdots \\
\mathrm{grad}_x f_{n}\left(x_{t}^n, y_{t}^1\right)
\end{array}\right], 
\bar{g}_{t}:=\frac{1}{n} \sum_{i=1}^{n} \mathrm{grad}_x f_{i}\left(x_{t}^i, y_t^i\right), \quad \bar{\mathbf{g}}_{t}:=\mathbf{1}_{n} \otimes \bar{g}_{t} \nonumber
\end{align}

we have following inequality:
% 1. Successive gradient error:
\begin{align}
&\left\|\mathbf{g}_{t+1}-\mathbf{g}_{t}\right\| \leq 2 \alpha L \left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\| + \beta L\left\|\mathbf{u}_{t}\right\| + L\|y_{t+1} - y_t\|  \label{eq:77}\\
% 2. Successive tracking error:
&\left\|\mathbf{u}_{t+1} - \bar{\mathbf{g}}_{t+1}\right\| \leq \sigma_{2}^{t}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\| + \left\|\mathbf{g}_{t+1} - \mathbf{g}_{t}\right\| \label{eq:78} \\
% 3. Successive consensus error: for $\rho_{k}=\sqrt{1-\gamma_{t} \alpha} \in(0,1)$,
&\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\| \leq \rho_{t}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\| + \beta\left\|\mathbf{u}_{t}\right\| \label{eq:79}
\end{align}

\begin{proof}
We firstly discuss about the proof of  \eqref{eq:77}
\begin{align}
\left\|\mathbf{g}_{t+1}-\mathbf{g}_{t}\right\| \leq& L\|x_{t+1} - x_t\| + L\|y_{t+1} - y_t\| \nonumber\\
\leq& \alpha L\|\mathrm{grad} J^k(x_t) \| + \beta L\|w_t \| + L\|y_{t+1} - y_t\| \nonumber\\
\leq& 2 \alpha L \left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\| + \beta L\left\|\mathbf{u}_{t}\right\| + L\|y_{t+1} - y_t\| 
\end{align}

% Under the same conditions of Fact B.1, if $\mathbf{x}_{t} \in \mathcal{N}$ and
% $$
% x_{t+1}^i = \mathcal{R}_{x_{t}^i}\left(-\alpha \operatorname{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right)+\beta v_{i, k}\right), \quad \forall i \in[n],
% $$
% where $w_{t}^i \in \mathrm{T}_{x_{i, k}} \mathcal{M}$, the following holds
% $$
% \left\|\mathbf{x}_{k+1}-\overline{\mathbf{x}}_{k+1}\right\|_{F} \leq \rho_{t}\left\|\mathbf{x}_{k}-\overline{\mathbf{x}}_{k}\right\|_{F}+\beta_{k}\left\|\mathbf{v}_{k}\right\|_{F}
% $$

For the \eqref{eq:78}, 
\begin{align} 
\|\mathbf{u}_{t+1} - \bar{\mathbf{g}}_{t+1} \| &= \|(\mathbf{I} - \frac{\mathbf{1} \mathbf{1}^{\top}}{n}) \otimes  \mathbf{u}_{t + 1} \| \nonumber\\ 
&= \|(\mathbf{I} - \frac{\mathbf{1} \mathbf{1}^{\top}}{n}) \otimes \left[\left(W^{k} \otimes \mathbf{I} \right) \mathbf{u}_{t} + \mathbf{g}_{t+1} -\mathbf{g}_{t}\right]\| \nonumber\\ 
&= \|(W^{k} - \frac{\mathbf{1} \mathbf{1}^{\top}}{n} ) \otimes  \mathbf{u}_{t}\|+ \|(\mathbf{I} - \frac{\mathbf{1} \mathbf{1}^{\top}}{n}) (\mathbf{g}_{t+1} - \mathbf{g}_{t}) \| \nonumber\\
&\leq \sigma_{2}^{t}\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\left\| + \right\| \mathbf{g}_{t+1} - \mathbf{g}_{t} \| 
\end{align}
For the proof of \eqref{eq:79}, by the definition of IAM, we have
\begin{align}
\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\|^{2} \leq& \left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t}\right\|^{2} \nonumber\\
=& \sum_{i=1}^{n}\left\|\mathcal{R}_{x_{t}^i}\left(-\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) - \beta_{t} w_{t}^i\right) - \hat{x}_{t}\right\|^{2} \nonumber\\
\leq& \sum_{i=1}^{n}\left\|x_{t}^i - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) - \beta_{t} w_{t}^i - \hat{x}_{t}\right\|^{2} \nonumber
\end{align}
Then we have
\begin{align}
\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\| &\leq \left\|\mathbf{x}_{t}-\alpha \mathrm{grad} J^{k}\left(\mathbf{x}_{t}\right)-\hat{\mathbf{x}}_{t} + \beta_{t} \mathbf{w}_{t}\right\| \nonumber\\
&\leq \left\|\mathbf{x}_{t}-\alpha \mathrm{grad} J^{k}\left(\mathbf{x}_{t}\right)-\hat{\mathbf{x}}_{t}\right\| + \beta_{t}\left\|\mathbf{w}_{t}\right\| \nonumber\\
&\leq \rho_{t}\left\|\mathbf{x}_{t}-\bar{\mathbf{x}}_{t}\right\| + \beta_{t}\left\|\mathbf{w}_{t}\right\| \nonumber\\
&\leq \rho_{t}\left\|\mathbf{x}_{t}-\bar{\mathbf{x}}_{t}\right\| + \beta_{t}\left\|\mathbf{u}_{t}\right\| \nonumber
\end{align}
\end{proof}
\end{lemma}

Then we start the proof of Theorem \ref{thm:1}.
\begin{proof}
\vspace*{-6pt}
\begin{align} 
\Phi\left(\hat{x}_{t+1}\right) - \Phi\left(\hat{x}_{t}\right) &\leq \left\langle\mathrm{grad} \Phi \left(\hat{x}_{t}\right), \hat{x}_{t+1} - \hat{x}_{t}\right\rangle + \frac{L_{\Phi}}{2} \left\|\hat{x}_{k+1} - \hat{x}_{k}\right\|^{2} \nonumber \\
& \leq \left\langle\bar{g}_{t}+ \mathrm{grad} \Phi\left(\hat{x}_{t}\right) - \mathrm{grad}_x F\left(\hat{x}_{t}, \bar{y}_t\right) + \mathrm{grad}_x F\left(\hat{x}_{t}, \bar{y}_t \right) - \bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{t}\right\rangle + \frac{L_{\Phi}}{2}\left\|\hat{x}_{t+1}-\hat{x}_{t}\right\|^{2} \nonumber\\
&\leq  \left\langle \bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{t}\right\rangle +  \eta \|\mathrm{grad} \Phi(\hat{x}_{t}) - \mathrm{grad}_x F\left(\hat{x}_{t}, \bar{y}\right)\|^2 + \eta \|\mathrm{grad}_x F\left(\hat{x}_{t}, \bar{y}\right) - \bar{g}_{t}\|^{2} + (\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2})\left\|\hat{x}_{t+1}-\hat{x}_{t}\right\|^{2}
\nonumber\\
& \leq \left\langle \bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{k}\right\rangle + \eta L^2 \|\bar{y}_t - y_t^{*} \|^2 + \frac{2 \eta L^2}{n} \left\|\mathbf{x}_{t}- \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 \eta L^2}{n} \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  (\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2}) \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber
\end{align}
where the last inequality holds by assumption \ref{ass:1} and the inequality that 
\begin{align}
\left\|\mathrm{grad} F\left(\hat{x}_{t}, \bar{y}_t\right) - \bar{g}_{t}\right\|^{2} \leq \frac{1}{n} \sum_{i=1}^{n}\left\|\mathrm{grad} f_i\left(\hat{x}_{t}, \bar{y}_t\right) - \mathrm{grad} f_{i}\left(x_{t}^i, y_t^i\right)\right\|^{2} \leq \frac{2L^{2}}{n}[\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \left\|\mathbf{y}_{t}-\bar{\mathbf{y}}_{t}\right\|^{2}]
\end{align}
For the first term, we have
\begin{align} \label{eq:85}
\left\langle\bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{t} \right\rangle &= \left\langle\bar{g}_{t}, \hat{x}_{t+1} - \bar{x}_{t+1} + \hat{x}_{t} -\bar{x}_{t}\right\rangle + \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle \nonumber\\
& \leq \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} + \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle
\end{align}
Recall that 
\begin{align}
\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \frac{3 \eta^2}{4}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+\frac{25 \eta}{6 \mu}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\end{align}
Combing the above inequalities, we have 
\begin{align}
&\Phi(\hat{x}_{t+1}) - \Phi(\hat{x}_{t}) + \frac{8L}{\mu \eta} [\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2}] \nonumber \\
\leq &  \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
&+ \frac{2 \eta L^2}{n} \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 \eta L^2}{n} \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  (\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2}) \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - \frac{6 \eta L}{\mu}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+\frac{67 L^3}{ \mu^2 n} [ \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} ]
 + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\nonumber\\
\leq & \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{ \mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{ \mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} 
\end{align}
Let $H_t = \Phi(\hat{x}_t) + \frac{8L}{\mu \eta} \left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} + \frac{ Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t\|^2 + \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2$ and based on lemma \ref{lem:6}
\begin{align} \label{eq:88}
& H_{t+1} - H_t \nonumber\\ 
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 -[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 \nonumber\\
&+ (1 + \frac{1}{c_0}) \frac{\eta Q}{n} \|\nabla_y F(x_{t+1}, y_{t+1}) - \nabla_y F(x_{t}, y_{t}) \|^2 \nonumber\\
% \leq &  
% \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{v}_t\right\|^{2} \nonumber\\
% &+ [\frac{2 \eta L^2}{n} + \frac{25 \eta L^2}{3 \mu n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{25 \eta L^2}{3 \mu n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber\\
% &- [1 - (1 + c_0)\lambda^2] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 -[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 \nonumber\\
% &+ (1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n}[ \|\mathbf{x}_{t+1} - \mathbf{x}_t \|^2 + 8\left\|\left(\mathbf{y}_{t-1} -  \bar{\mathbf{y}}_{t-1}\right)\right\|^{2} + 4 \eta^{2}\left\|\mathbf{v}_{t-1} - \bar{\mathbf{v}}_{t-1}\right\|^{2} + 4 \eta^{2} n\left\|\bar{v}_{t-1}\right\|^{2} ] \nonumber \\
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{v}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 -[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 \nonumber\\
&+ (1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n}[ \|\mathbf{x}_{t+1} - \mathbf{x}_t \|^2 + 8\left\|\left(\mathbf{y}_{t} -  \bar{\mathbf{y}}_{t}\right)\right\|^{2} + 4 \eta^{2}\left\|\mathbf{v}_{t} - \bar{\mathbf{v}}_{t}\right\|^{2} + 4 \eta^{2} n\left\|\bar{v}_{t}\right\|^{2}] \nonumber \\
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n}  \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{6L^2 \eta Q}{n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n} \|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 6L^2 \eta Q] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 8L^2 \eta^3 Q - 12C_8 L^2 \eta^2]\left\|\bar{v}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24C_8 L^2}{Q}] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 
\end{align}
Then, for the first term, we have
\begin{align} \label{eq:89}
&\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t}\right\rangle \nonumber\\
=&\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t} - \beta \bar{g}_{t} + \beta \bar{g}_{t}\right\rangle \nonumber\\
=& -\beta\left\|\bar{g}_{t}\right\|^{2} + \langle \bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n} [x_{t+1}^i - (x_{ t}^i - \beta w_{t}^i - \alpha \mathrm{grad} J_{i}^{k}(\mathbf{x}_{t}))]\rangle +\langle\bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n}\left[\beta\left(u_{t}^i - w_{t}^i\right) - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right)\right]\rangle .
\end{align}
For the last term in \eqref{eq:89}
\begin{align}
&\langle\bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n} \beta\left(w_{t}^i-u_{t}^i\right)-\alpha \mathrm{grad} J_{i}^{k} \left({x}_{t}^i\right)\rangle \nonumber\\
\leq & \frac{\beta}{n} \sum_{i=1}^{n}\left\langle \bar{g}_{t} - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_{t}^i\right), w_{t}^i - u_{t}^i\right\rangle + \frac{2 \alpha}{n}\left\|\bar{g}_{t}\right\| \cdot\left\|\mathbf{x}_{t}-\overline{\mathbf{x}}_{t}\right\|^{2} \nonumber \\
\leq& \frac{1}{4 n L} \sum_{i=1}^{n}\left\|\bar{g}_{t} - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_{t}^i\right)\right\|^{2}+\frac{\beta^{2} L}{n} \sum_{i=1}^{n}\left\|\mathcal{P}_{N_{x_{i, k}}} u_{t}^i\right\|^{2} + \frac{2 \alpha D}{n}\left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\|^{2} \nonumber\\
\leq& \frac{1}{4 n^{2} L} \sum_{i=1}^{n} \sum_{j=1}^{n}\left\|\mathrm{grad}_x f_{j}\left(x_{t}^j, y_t^j\right) - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_t^i\right)\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{u}_{t}\right\|^{2}+\frac{2 \alpha D}{n}\left\|\mathbf{x}_{t}-\bar{\mathbf{x}}_{t}\right\|^{2} \nonumber\\
\leq & \frac{L+2 \alpha D}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2}+  \frac{\beta^{2} L}{n}\left\|\mathbf{u}_{t}\right\|^{2},
\end{align}
where the first inequality holds by the Cauchy-Schwartz inequality, $w_{t}^i-u_{t}^i \in N_{x_t^i} \mathcal{M}$ and lemma \ref{lem:3} (3). Therefore,
\begin{align}
&\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t}\right\rangle \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2} + \left\langle\bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n}\left[x_{t+1}^i - \left(x_{t}^i - \beta u_{t}^i - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}^i\right)\right)\right]\right\rangle + \frac{L +2 D \alpha}{n}\left\|\mathbf{x}_{k}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L }{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq&  -\beta\left\|\bar{g}_{t}\right\|^{2}+\frac{D}{n} \sum_{i=1}^{n}\left\|x_{t}^i  - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) - \beta u_{t}^i - x_{t+1}^i\right\| + \frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{M D}{n} \sum_{i=1}^{n}\left\|\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{k}\right)+\beta u_{t}^i\right\|^{2} + \frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{2 M D \alpha^{2}}{n}\left\|\mathrm{grad} J^{t}\left(\mathbf{x}_{k}\right)\right\|_{\mathrm{F}}^{2}+\frac{2 M D \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2}+\frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{8 M D \alpha^{2}+2 D \alpha + L}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left(2 M D+L\right) \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} 
\end{align}
where the third inequality holds by Lemma \ref{lem:1} and the last inequality holds by Lemma \ref{lem:3} (2)

For the terms in \eqref{eq:88}, based on the Lemma \ref{lem:3} (3), we have
\begin{align}
&\left\|\bar{x}_{t}-\hat{x}_{t}\right\|^{2}+\left\|\bar{x}_{t+1}-\hat{x}_{t+1}\right\|^{2} \nonumber\\
\leq& \frac{4 r}{n^{2}}\left(\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{4} + \left\|\mathbf{x}_{t + 1}-\hat{\mathbf{x}}_{t+1}\right\|^{4}\right) 
\end{align}
% where the inequality holds by Lemma \ref{lem:5}
% We then obtain
% \begin{align}
% b_{2} \leq \frac{4 r}{n^{2} \beta^{2} L_{G}}\left(\left\|\mathbf{x}_{k}-\overline{\mathbf{x}}_{k}\right\|_{\mathrm{F}}^{4}+\left\|\mathbf{x}_{k+1}-\overline{\mathbf{x}}_{k+1}\right\|_{\mathrm{F}}^{4}\right) .
% \end{align}

Thirdly, Based on Lemma \ref{lem:8} and $\alpha \leq 1 / M$ yields
\begin{align}
\left\|\hat{x}_{t}-\hat{x}_{t+1}\right\| \leq \frac{1}{1-2 \delta_{1}^{2}}\left[\frac{10 \alpha}{n}\left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\|^{2} + \frac{2 M \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2}+\beta\left\|\bar{w}_{t}\right\|\right] .
\end{align}
Then, if we choose $\beta$ to let  $\beta\left\|\mathbf{u}_{t}\right\| \leq \frac{\alpha \delta_{1}}{2}$ that
\begin{align}
& \|\hat{x}_{t+1} - \hat{x}_{t} \|^2 \leq \left(\frac{2}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{10 \alpha}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 M \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2}\right]^{2} + \frac{2}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left\|\bar{w}_{t}\right\|^{2}\right) \nonumber\\
\leq & \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{4} + \frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2}\right]+\frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{u}_{t}\right\|^{2}+\left\|\bar{w}_{t}-\bar{u}_{t}\right\|_{\mathrm{F}}^{2}\right) \nonumber\\
\leq & \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{4}+\frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2}\right]+\frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{u}_{t}\right\|^{2}\right)
\end{align}

where we use $\bar{u}_{t}=\bar{g}_{t}$ and $\left\|\bar{u}_{t} - \bar{w}_{t}\right\|^{2} \leq \frac{1}{n}\left\|\mathcal{P}_{N_{x_{i, k}}} u_{i, k}\right\|^{2} \leq \frac{1}{n}\left\|\mathbf{u}_{t}\right\|^{2}$. It follows from   that
\begin{align}
\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq 25 C_{1} D^{2} \beta^{2} \leq \frac{C_{1} \alpha^{2} \delta_{1}^{2}}{4}
\end{align}
where we use $\beta \leq \frac{\alpha \delta_{1}}{10 D}$. Therefore, we get
\begin{align}
\frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} \leq \frac{100 r D^{2} C_{1}}{n L}\left(\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\|^{2}\right)
\end{align}
and
\begin{align}
\|\hat{x}_{t+1} - \hat{x}_{t} \|^2 
&\leq  \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{4}+\frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2}\right]+\frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{u}_{t}\right\|^{2}\right) \nonumber\\
&\leq \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{25 \alpha^{4} C_1 \delta_1^2}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left( \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2}\right]+\frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{u}_{t}\right\|^{2}\right) \nonumber\\
&\leq \frac{101 \alpha^{4} C_1 \delta_1^2}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{ ( 5 \delta_{1}^2 + 5 )\beta^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{9}{2} \beta^{2}\left\|\bar{g}_{t}\right\|^{2}
\end{align}

where we use $\alpha \leq \frac{1}{M}$ and $\frac{1}{\left(1-2 \delta_{1}^{2}\right)^{2}} \leq 1.002$. 

Therefore,
\begin{align} \label{eq:98}
&H_{t+1} - H_t \nonumber\\
\leq& 
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n}  \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{6L^2 \eta Q}{n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n} \|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 6L^2 \eta Q] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 8L^2 \eta^3 Q - 12C_8 L^2 \eta^2]\left\|\bar{v}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24C_8 L^2}{Q}] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 
\nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{8 M D \alpha^{2}+2 D \alpha + L}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left(2 M D+L\right) \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} \nonumber\\
&+ \frac{100 r D^{2} C_{1}}{n L}\left(\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\|^{2}\right) - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n}  \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2  \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{6L^2 \eta Q}{n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n} \|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+ [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 6L^2 \eta Q][\frac{101 \alpha^{4} C_1 \delta_1^2}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{ ( 5 \delta_{1}^2 + 5 )\beta^{2}}{ n}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{9}{2} \beta^{2}\left\|\bar{g}_{t}\right\|^{2}] \nonumber\\
&- [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 8L^2 \eta^3 Q - 12C_8 L^2 \eta^2]\left\|\bar{v}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24C_8 L^2}{Q}] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 
\nonumber\\
\leq& - [\beta - \frac{\beta^2 (L + 9C_2)}{2} ] \left\|\bar{g}_{t}\right\|^{2}  + \frac{\left(2 M D+L + C_2( 5 \delta_{1}^2 + 5 )\right) \beta^{2}}{n}\left\|\mathbf{u}_{t}\right\|^{2} - \frac{3 C_8 L^2}{n}  \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{100 r D^{2} C_{1}}{n L} + \frac{2 \eta L^2}{n} + \frac{67 L^2}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{6L^2 \eta Q}{n} + C_2\frac{101 \alpha^{4} C_1 \delta_1^2}{n} + \frac{8 M D \alpha^{2}+2 D \alpha + L}{n}] \left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2  \nonumber\\
&+ [(1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n} + \frac{100 r D^{2} C_{1}}{n L}] \|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  \nonumber \\
&- [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 8L^2 \eta^3 Q - 12C_8 L^2 \eta^2]\left\|\bar{v}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{L}{2Q} -   [\frac{2 \eta L^2}{Q} + \frac{25 \eta L^2}{3 \mu Q}]  - \frac{24C_8 L^2}{Q}] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \|\mathbf{v}_t - \bar{\mathbf{v}}_t \|^2 
\end{align}

where $C_2 = [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 6L^2 \eta Q]$

We need to make sure $[\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 8L^2 \eta^3 Q - 12C_8 L^2 \eta^2] \geq 0, [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{L}{2Q} -   [\frac{2 \eta L^2}{Q} + \frac{25 \eta L^2}{3 \mu Q}]  - \frac{24 C_8 L^2}{Q}] \geq 0$and $[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12C_8 L^2 \eta}{Q}] \geq 0$.
Let $c_0 = \frac{1}{\lambda} - 1, Q = 48 C_8 L^2$ and $\eta \leq \min \{\frac{1}{8 C_8 L^2}, \frac{1}{12L^2(1 + \frac{1}{c_0})} \}$
Recall 
\begin{align}
\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\| \leq \rho_{k}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\| + \beta\left\|\mathbf{u}_{t}\right\| .
\end{align}
We apply the Lemma \ref{lem:7}
\begin{align} \label{eq:100}
\frac{1}{n} \sum_{t=0}^{T}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq C_3 \frac{\beta^{2}}{n} \sum_{t=0}^{T}\left\|\mathbf{u}_{t}\right\|^{2},  
\end{align}

where $C_3 = \frac{2}{\left(1-\rho_{k}\right)^{2}}$. Telescoping \eqref{eq:98}, we have
\begin{align} \label{eq:101}
& H_{T} - H_0 \nonumber\\
\leq& - [\beta - \frac{\beta^2 (L + 9C_2)}{2} ]\sum_{t=0}^{T-1} \left\|\bar{g}_{t}\right\|^{2} + \frac{C_5}{n} \beta^2 \sum_{t=0}^{T}\left\|\mathbf{u}_{t}\right\|
+ \frac{C_6}{n} \sum_{t=0}^{T-1}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{C_7}{n} \sum_{t=1}^{T}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} - L \sum_{t=0}^{T-1}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
&- \frac{3 C_8 L^2}{n}  \sum_{t=0}^{T-1}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
\leq & - [\beta - \frac{\beta^2 (L + 9C_2)}{2} ]\sum_{t=0}^{T-1} \left\|\bar{g}_{t}\right\|^{2} + (C_5 + C_6 C_3 + C_7 C_3)
\frac{\beta^{2}}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{C_3 C_7\beta^{2}\left\|\mathbf{u}_{T}\right\|^{2}}{n}  - L \sum_{t=0}^{T-1} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber \\
&- \frac{3 C_8 L^2}{n}  \sum_{t=0}^{T-1}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
\leq& -\frac{\beta}{2} \sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2} + \frac{(C_5 + C_6 C_3 + C_7 C_3)\beta^{2}}{n} \sum_{t=0}^{T-1} \left\|\mathbf{u}_{t}\right\|^{2} + C_4 - \frac{L}{n} \sum_{t=0}^{T-1}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n} \sum_{t=0}^{T-1} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 
\end{align}

where we use $\beta \leq \min \left\{\frac{1}{L + 9 C_2 }, \frac{\alpha \delta_{1}}{10 D}\right\}, \beta^{2}\left\|\mathbf{u}_{T+1}\right\|^{2} \leq 25nD^{2} \beta^{2} \leq \frac{\delta_{1}^{2} \alpha^{2} n}{4}$ and $C_4=\frac{C_3 C_7 \delta_{1}^{2} \alpha^{2}}{4} $
% 
in the last inequality.
We are going to associate $\left\|\bar{g}_{t}\right\|^{2}$ with $\left\|\mathbf{u}_{t}\right\|^{2}$. 
We have the fact that 
\begin{align}
\left\|\mathbf{u}_{t}\right\| \leq\left\|\mathbf{u}_{t}-\bar{\mathbf{g}}_{t}\right\| + \left\|\bar{\mathbf{g}}_{t}\right\|
\end{align}
Then, we get
\begin{align}
-\sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2}= -\frac{1}{n} \sum_{t=0}^{T-1}\left\|\bar{\mathbf{g}}_{t}\right\|^{2} \leq \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\|^{2} - \frac{1}{2 n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2}
\end{align}
where $\bar{\mathbf{g}}_{t}:=\mathbf{1}_{n} \otimes \bar{g}_{t}$. With Lemma \ref{lem:10}
\begin{align}
\left\|\mathbf{u}_{t+1} - \bar{\mathbf{g}}_{t+1}\right\| \leq \sigma_{2}^{t}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\| + \left\|\mathbf{g}_{t+1} - \mathbf{g}_{t}\right\|
\end{align}
and Lemma \ref{lem:7}, we have 
\begin{align}
\frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\|^{2} &\leq C_8 \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{g}_{t+1} - \mathbf{g}_{t}\right\|^{2} \nonumber\\
% + C_9 
&\leq C_8 \frac{1}{n} \sum_{t=0}^{T-1}(12 \alpha^{2} L^{2}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + 3 \beta^{2} L^{2}\left\|\mathbf{u}_{t}\right\|^{2} + 3L^2 \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 )  \nonumber\\
&\leq \left(12 \alpha^{2} C_3 C_8 + 3 C_8\right) L^{2} \beta^{2} \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + 3L^2 C_8 \frac{1}{n} \sum_{t=0}^{T-1} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber \\
% + 12 \alpha^{2} C_4 C_8 L^{2}  
% &\leq\left(8 \tilde{C}_{0}+\frac{1}{2} \tilde{C}_{2}\right) \alpha \delta_{1} L_{G} \beta \frac{1}{n} \sum_{k=0}^{K}\left\|\mathbf{y}_{k}\right\|_{\mathrm{F}}^{2} + 3L^2 C_8 \frac{1}{n} \sum_{t=0}^{T} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 + 12 \alpha^{2} \tilde{C}_{1} \tilde{C}_{2} L_{G}^{2}+\tilde{C}_{3}
\end{align}
where  $C_8 = \frac{2}{\left(1-\sigma_{2}^{t}\right)^{2}}$ and the first inequality holds by Lemma \ref{lem:10} and the second inequality holds by \eqref{eq:100}. Combing the above inequalities, we have
% and $C_9 = \frac{2}{1-\sigma_{2}^{2 t}} \cdot \frac{1}{n}\|\mathbf{u}_{0}-\bar{\mathbf{g}}_{0}\|^ {2}$. 
% The last line is due to $\beta \leq \frac{\alpha \delta_{1}}{5 L}$ and $\alpha^{2} \tilde{C}_{2} \leq \tilde{C}_{2} \leq$ $\frac{2}{\left(1-\frac{1}{2 \sqrt{n}}\right)^{2}} \leq 5$. 
\begin{align}
-\sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2} \leq \left[\left(12 \alpha^{2} C_3 C_8 + 3 C_8\right) L^{2} \beta^{2} - \frac{1}{2}\right] \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + 3L^2 C_8 \frac{1}{n} \sum_{t=0}^{T-1} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 
% +  12 \alpha^{2} C_4 C_8 L^{2} + C_9
\end{align}

Hence, it follows from \eqref{eq:101} that
\begin{align} \label{eq:107}
& H_{T} - H_0 \nonumber\\
\leq & - \frac{\beta}{2} \sum_{t=0}^{T-1} \left\|\bar{g}_{t}\right\|^{2} + (C_5 + C_6 C_3 + C_7 C_3) \frac{\beta^{2}}{n} \sum_{t=0}^{T-1} \left\|\mathbf{u}_{t}\right\|^{2} + C_{4} - \frac{L}{n}\sum_{t=0}^{T-1} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n} \sum_{t=0}^{T-1} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2  \nonumber\\
\leq & - \frac{\beta}{2}[ \frac{1}{2} - \left(12 \alpha^{2} C_3 C_8 + 3 C_8\right) L^{2} \beta^{2} - 2(C_5 + C_6 C_3 + C_7 C_3)\beta]  
\frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + C_{4} - \frac{L}{n}\sum_{t=0}^{T-1} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
\leq & - \frac{\beta}{10n}  \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + C_{4} - \frac{L}{n}\sum_{t=0}^{T-1} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2
\end{align}
where $ \beta \leq \beta_0 = \min \{\frac{1}{5\sqrt{(12 \alpha^{2} C_3 C_8 + 3 C_8)L^2}}, \frac{1}{10(C_5 + C_6 C_3 + C_7 C_3)} \}$

Then, we get
\begin{align}
\frac{\beta}{10} \sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2} \leq \frac{\beta}{10} \cdot \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} \leq H_0 - H_{T} + C_{4} - \frac{L}{n}\sum_{t=0}^{T-1} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2
\end{align}
\begin{align}
\frac{1}{T} \sum_{t=0}^{T - 1}[\left\|\bar{g}_{t}\right\|^{2} + \frac{10L}{n \beta} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \leq \frac{10(H_0 - H_{T}  + C_{4})}{T \beta} 
\end{align}
% $\tilde{C}_{4}=\left(8 \alpha^{2} \tilde{C}_{1} \tilde{C}_{2} L_{G}^{2}+\tilde{C}_{3}\right) \frac{\beta}{2}=\mathcal{O}\left(\frac{r \delta_{1}^{2} L_{G}}{\left(1-\sigma_{2}^{t}\right)^{2}}\right)$ and $f^{*}=\min _{x \in \operatorname{St}(d, r)} f(x)$. This implies
Combing the \eqref{eq:100} and \eqref{eq:107}, we also have 
\begin{align}
\frac{1}{T} \sum_{i=0}^{T-1}[\frac{1}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + 10\beta C_3 L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \leq \frac{10 \beta( H_0 - H_{T} + C_{4}) C_3 }{T} .  
\end{align}

So,
\begin{align}
\frac{1}{T} \sum_{i=0}^{T-1} \mathfrak{M}_t &= \frac{1}{T} \sum_{i=0}^{T}[\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{L}{n} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \nonumber\\
&\leq 
\frac{1}{T} \sum_{i=0}^{T}[ \left\|\bar{g}_{t}\right\|^{2} + \frac{10L}{n \beta} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 + \frac{1}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{10\beta C_3 L}{n} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \nonumber\\
&\leq \frac{10(H_0 - H_{T} + C_{4})}{T \beta}  + \frac{10 \beta( H_0 - H_{T} + C_{4}) C_3}{T} .  
\end{align}
where we use the fact that $C_3 \geq 1$
\end{proof}

\subsection{Convergence Analysis of DRSGDA Algorithms}
In the Algorithms\ref{alg:2}, we use the $\{\underline{u}_t\}$ and $\{\underline{v}_t\}$ to track the gradient estimators. To facilitate our analysis, we also define “virtual sequences” $\{u_t\}$ and $\{v_t\}$ as in the algorithm \ref{alg:1}.
\begin{lemma}  (Bounded Variance)
Under assumption \ref{ass:4} and the iterates $\left\{\mathbf{v}_t\right\}$ are generated by algorithm \ref{alg:2}, then we have  
\begin{align}
\mathbb{E}\left\|\mathbf{v}_t - \underline{\mathbf{v}}_t\right\|^{2} \leq \frac{\tilde{\eta} \sigma^{2}}{B}  \\
\mathbb{E}\left\|\mathbf{u}_t - \underline{\mathbf{u}}_t\right\|^{2} \leq \frac{\tilde{\eta} \sigma^{2}}{B}
\end{align}
where $\tilde{\eta} = \frac{8 n \sigma^2}{(1 - \lambda^2)^2 }$
\begin{proof}
we have
\begin{align}
\mathbb{E}\|\mathbf{v}_{t+1} - \underline{\mathbf{v}}_{t+1}\|^2 &=  
\mathbb{E}\|\mathbf{W}\left(\mathbf{v}_{t} - \underline{\mathbf{v}}_t\right) + [\nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}; \mathcal{B}_{t+1}\right) - \nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}\right) - \nabla_y F\left(\mathbf{x}_{t}, \mathbf{y}_{t}; \mathcal{B}_{t}\right) + \nabla_y F\left(\mathbf{x}_{t}, \mathbf{y}_{t}\right)] \|^2 \nonumber\\
&\leq \frac{1 + \lambda}{2}\mathbb{E}\|\mathbf{W}\left(\mathbf{v}_{t} - \underline{\mathbf{v}}_t\right)]\|^2 + \frac{4}{1 - \lambda^2}\mathbb{E}[\|\nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}; \mathcal{B}_{t+1}\right) - \nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}\right)\| \nonumber\\
&+ \|\nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}; \mathcal{B}_{t+1}\right) - \nabla_y F\left(\mathbf{x}_{t+1}, \mathbf{y}_{t+1}\right)\|] \nonumber\\
&\leq \lambda^2 \mathbb{E}\|\mathbf{v}_{t} - \underline{\mathbf{v}}_t]\|^2 + \frac{8 n \sigma^2}{1 - \lambda^2  B} 
\end{align}
As the $\mathbb{E}\|\mathbf{v}_{0} - \underline{\mathbf{v}}_0]\|^2 = \frac{n \sigma^2}{B} $, we have 
\begin{align}
\mathbb{E}\|\mathbf{v}_{t+1} - \underline{\mathbf{v}}_{t+1}\|^2 \leq \frac{8 n \sigma^2}{(1 - \lambda^2)^2  B} 
\end{align}
\end{proof}
\end{lemma}
\begin{lemma} \label{lem:12}
Under assumptions \ref{ass:1}, and let $x_t \in \mathcal{N}$, $k \geq \lceil log_{\lambda_2} ( \frac{1}{2\sqrt{n}} ) \rceil$, then $\|v_t^i \| \leq 5D \forall i \in [n]$. If $x_t \in N$ and $\forall t \geq 0$. And following holds:
\begin{align} \label{eq:77}
\frac{1}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq  C_{1}(5D + \tilde{\gamma} \sigma)^2 \beta^{2}, t \geq 0 .
\end{align}

\begin{proof}
Following the Lemma \ref{lem:9}, we have
\begin{align}
\left\|\underline{u}_{t+1}^i - \bar{g}_{t}\right\| \leq 4D 
\end{align}
Hence, $\mathbb{E}\left\| u_{t+1}^i\right\| \leq \left\|u_{t+1}^i - \underline{u}_{t+1}^i\right\| + \left\|\underline{u}_{t+1}^i - \bar{g}_{t}\right\| + \left\|\bar{g}_{t}\right\| \leq 5 D + \tilde{\gamma} \sigma$. 
Following the Lemma \ref{lem:9}, there exists some $C_{1}=\mathcal{O}\left(\frac{1}{\left(1-\rho_{k}\right)^{2}}\right)$ that is independent of $L$ and $D$ such that
\begin{align}
\frac{1}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq C_{1}(5D + \tilde{\gamma} \sigma)^2 \beta^{2}, t \geq 0 \nonumber
\end{align}
\end{proof}
\end{lemma}
Then we start the proof of Theorem \ref{thm:2}.
\vspace*{-10pt}
\begin{proof}
\begin{align}
\Phi\left(\hat{x}_{t+1}\right) - \Phi\left(\hat{x}_{t}\right) &\leq \left\langle\mathrm{grad} \Phi \left(\hat{x}_{t}\right), \hat{x}_{t+1} - \hat{x}_{t}\right\rangle + \frac{L_{\Phi}}{2} \left\|\hat{x}_{k+1} - \hat{x}_{k}\right\|^{2} \nonumber \\
& \leq \left\langle \bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{k}\right\rangle + \eta L^2 \|\bar{y}_t - y_t^{*} \|^2 + \frac{2 \eta L^2}{n} \left\|\mathbf{x}_{t}- \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 \eta L^2}{n} \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  (\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2}) \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber
\end{align}
For the first term,
\begin{align}
\left\langle\bar{g}_{t}, \hat{x}_{t+1} - \hat{x}_{t} \right\rangle &= \left\langle\bar{g}_{t}, \hat{x}_{t+1} - \bar{x}_{t+1} + \hat{x}_{t} -\bar{x}_{t}\right\rangle + \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle \nonumber\\
& \leq \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} + \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle
\end{align}
Based on Lemma \ref{lem:5}
% \begin{align}
% \mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \mathbb{E}\left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2} \leq &-\frac{\eta \mu}{4}\mathbb{E}\left\|y_{t}-y^{*}\left(\hat{x}_{t}\right)\right\|^{2} - \frac{3 \eta^2}{4}\mathbb{E}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
% &+\frac{25 \eta}{6 \mu}\mathbb{E}\left\|\nabla_{y} F\left(\hat{x}_{t}, \bar{y}_{t}\right) - \bar{v}_{t}\right\|^{2} + \frac{5 \kappa^{2}}{ \mu \eta }\mathbb{E}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
% \end{align}
we have 
\begin{align}
&\mathbb{E}[\Phi(\hat{x}_{t+1})] - \mathbb{E}[\Phi(\hat{x}_{t})] + \frac{8L}{\mu \eta} [\mathbb{E}\left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} - \mathbb{E}\left\|\bar{y}_{t} - y^{*}\left(\hat{x}_{t}\right)\right\|^{2}] \nonumber \\
\leq &  \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
&+ \frac{2 \eta L^2}{n} \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 \eta L^2}{n} \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  (\frac{1}{2 \eta} + \frac{ L_{\Phi}}{2}) \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - \frac{6 \eta L}{\mu}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+\frac{67 L^3}{ \mu^2 n} [ \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} ]
 + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2}
\nonumber\\
\leq & \left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{ \mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} 
\end{align}

Let $H_t = \Phi(\hat{x}_t) + \frac{8L}{\mu \eta} \left\|\bar{y}_{t+1}-y^{*}\left(\hat{x}_{t+1}\right)\right\|^{2} + \frac{ Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t\|^2 + \frac{\eta Q}{n} \|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2$, we have
\begin{align}
& \mathbb{E}[H_{t+1}] - \mathbb{E}[H_t] \nonumber\\
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{ \mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 -[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta] \frac{\eta Q}{n} \|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 \nonumber\\
&+ (1 + \frac{1}{c_0}) \frac{\eta Q}{n} \mathbb{E}\|\nabla_y F(x_{t+1}, y_{t+1}; \mathcal{B}_{t+1}) - \nabla_y F(x_{t}, y_{t};\mathcal{B}_{t}) \|^2 \nonumber\\
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{6 \eta L}{\mu}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t} -  \bar{\mathbf{y}}_{t}\right\|^{2} +  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 }] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 -[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta] \frac{\eta Q}{n} \|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 \nonumber\\
&+ (1 + \frac{1}{c_0}) \frac{6 L^2 \eta Q}{n}[ \|\mathbf{x}_{t+1} - \mathbf{x}_t \|^2 + 8\left\|\left(\mathbf{y}_{t} -  \bar{\mathbf{y}}_{t}\right)\right\|^{2} + 4 \eta^{2}\left\|\mathbf{\underline{v}}_{t} - \bar{\mathbf{\underline{v}}}_{t}\right\|^{2} + 4 \eta^{2} n\left\|\bar{\underline{v}}_{t}\right\|^{2}] +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}  \nonumber \\
&- \frac{3 C_8 L^2}{n}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 + \frac{3 C_8 L^2}{n}[8\| \mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\|^2 + 4 \eta^2\|\mathbf{\underline{v}}_{t} - \bar{\mathbf{\underline{v}}}_{t}\|^2 + 4 \eta^2 n \|\bar{\underline{v}}_t\|^2]\nonumber\\
\leq &  
\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{18 L^2 \eta Q}{n}] \left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{18 L^2 \eta Q}{n} \|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 18 L^2 \eta Q] \left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 24 L^2 \eta^3 Q - 12 C_8 L^2 \eta^2]\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24 C_8 L^2}{Q}] \frac{Q}{n} \|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8 L^2 \eta^{2} - \frac{12 C_8 L^2 \eta}{Q} ] \frac{\eta Q}{n} \|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 
\end{align}
Then, for the first term, we have $\mathbb{E}[\bar{g}_t] = \mathbb{E}[\bar{u}_t] = \frac{1}{n}  \mathbb{E}[\underline{u}_t^i]$ and
\begin{align}
&\mathbb{E}\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t}\right\rangle \nonumber\\
=&\mathbb{E}\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t} - \beta \bar{g}_{t} + \beta \bar{g}_{t}\right\rangle \nonumber\\
=& -\beta\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \mathbb{E}\langle \bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n} [x_{t+1}^i - (x_{ t}^i - \beta w_{t}^i - \alpha \mathrm{grad} J_{i}^{k}(\mathbf{x}_{t}))]\rangle  + \mathbb{E}\langle\bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n}\left[\beta\left(\underline{u}_{t}^i - w_{t}^i\right) - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right)\right]\rangle .
\end{align}
\begin{align}
&\left\langle\bar{g}_{t}, \frac{\beta}{n} \sum_{i=1}^{n}\left(\underline{u}_{t}^i - w_{t}^i\right)-\alpha \mathrm{grad} J_{i}^{k} \left({x}_{t}^i\right)\right\rangle \nonumber\\
\leq & \frac{\beta}{n} \sum_{i=1}^{n}\left\langle \bar{g}_{t} - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_{t}^i\right), \underline{u}_{t}^i - w_{t}^i\right\rangle + \frac{2 \alpha}{n}\left\|\bar{g}_{t}\right\| \cdot\left\|\mathbf{x}_{t}-\overline{\mathbf{x}}_{t}\right\|^{2} \nonumber \\
\leq& \frac{1}{4 n L} \sum_{i=1}^{n}\left\|\bar{g}_{t} - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_{t}^i\right)\right\|^{2}+\frac{\beta^{2} L}{n} \sum_{i=1}^{n}\left\|\mathcal{P}_{N_{x_{i, k}}} \underline{u}_{t}^i\right\|^{2} + \frac{2 \alpha D}{n}\left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\|^{2} \nonumber\\
\leq& \frac{1}{4 n^{2} L} \sum_{i=1}^{n} \sum_{j=1}^{n}\left\|\mathrm{grad}_x f_{j}\left(x_{t}^j, y_t^j\right) - \mathrm{grad}_x f_{i}\left(x_{t}^i, y_t^i\right)\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}+\frac{2 \alpha D}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} \nonumber\\
\leq & \frac{L+2 \alpha D}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} +  \frac{\beta^{2} L}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2},
\end{align}
where the first inequality holds by  that $w_{t}^i - \underline{u}_{t}^i \in N_{x_{t}^i} \mathcal{M}$.Therefore, 

\begin{align}
&\left\langle\bar{g}_{t}, \bar{x}_{t+1}-\bar{x}_{t}\right\rangle \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2} + \left\langle\bar{g}_{t}, \frac{1}{n} \sum_{i=1}^{n}\left[x_{t+1}^i - \left(x_{t}^i - \beta w_{t}^i - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}^i\right)\right)\right]\right\rangle + \frac{L +2 D \alpha}{n}\left\|\mathbf{x}_{k}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L }{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq&  -\beta\left\|\bar{g}_{t}\right\|^{2}+\frac{D}{n} \sum_{i=1}^{n}\left\|x_{t}^i  - \alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{t}\right) - \beta w_{t}^i - x_{t+1}^i\right\| + \frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{M D}{n} \sum_{i=1}^{n}\left\|\alpha \mathrm{grad} J_{i}^{k}\left(\mathbf{x}_{k}\right)+\beta w_{t}^i\right\|^{2} + \frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{2 M D \alpha^{2}}{n}\left\|\mathrm{grad} J^{t}\left(\mathbf{x}_{k}\right)\right\|_{\mathrm{F}}^{2}+\frac{2 M D \beta^{2}}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}+\frac{L + 2 D \alpha}{n}\left\|\mathbf{x}_{t} - \bar{\mathbf{x}}_{t}\right\|^{2} + \frac{\beta^{2} L}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber\\
\leq& - \beta\left\|\bar{g}_{t}\right\|^{2}+\frac{8 M D \alpha^{2}+2 D \alpha + L}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left(2 M D + L\right) \beta^{2}}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} 
\end{align}
From the Lemma \ref{lem:3} (3), we have
\begin{align}
&\left\|\bar{x}_{t} - \hat{x}_{t}\right\|^{2} + \left\|\bar{x}_{t+1} - \hat{x}_{t+1}\right\|^{2} \nonumber\\
\leq& \frac{4 r}{n^{2}}\left(\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{4} + \left\|\mathbf{x}_{t + 1} - \hat{\mathbf{x}}_{t+1}\right\|^{4}\right) 
\end{align}
% where the inequality holds by Lemma \ref{lem:5}
% We then obtain
% \begin{align}
% b_{2} \leq \frac{4 r}{n^{2} \beta^{2} L}\left(\left\|\mathbf{x}_{t}-\bar{\mathbf{x}}_{k}\right\|^{4}+\left\|\mathbf{x}_{k+1}-\overline{\mathbf{x}}_{t+1}\right\|^{4}\right) .
% \end{align}
Following  the Lemma \ref{lem:8}, we also have
\begin{align}
\left\|\hat{x}_{t}-\hat{x}_{t+1}\right\| \leq \frac{1}{1-2 \delta_{1}^{2}}\left[\frac{10 \alpha}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 M \beta^{2}}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}+\beta\left\|\bar{w}_{t}\right\|\right] .
\end{align}
Then, if we choose $\beta$ to let  $\beta \mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\| \leq \frac{\alpha \delta_{1}}{2}$,  then
\begin{align}
& \|\hat{x}_{t+1} - \hat{x}_{t} \|^2 \leq \left(\frac{2}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{10 \alpha}{n}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{2 M \beta^{2}}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}\right]^{2} + \frac{2}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left\|\bar{w}_{t}\right\|^{2}\right) \nonumber\\
\leq & \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{4} + \frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}\right] + \frac{6}{\left(1 - 2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{u}_{t}\right\|^{2} + \left\|\bar{w}_{t}-\bar{\underline{u}}_{t}\right\|^{2}+ \left\|\bar{\underline{u}}_{t} - \bar{u}_{t}\right\|^{2} \right) \nonumber\\
\leq & \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{4}+\frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}\right]+\frac{6}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{\underline{u}}_{t} \right\|^{2} + \left\|\bar{\underline{u}}_{t}-\bar{u}_{t}\right\|^{2} \right)
\end{align}
where we use $\bar{u}_{t}=\bar{g}_{t}$ and $\left\|\bar{w}_{t} - \bar{\underline{u}}_{t}\right\|^{2} \leq \frac{1}{n}\left\|\mathcal{P}_{N_{x_{t}^i}} u_{t}^i\right\|^{2} \leq \frac{1}{n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}$. It follows from .... that
\begin{align}
\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq C_{1}(\tilde{\gamma}\sigma+ 5D)^{2} \beta^{2} \leq \frac{C_{1} \alpha^{2} \delta_{1}^{2}}{4}
\end{align}
where we use $\beta \leq \frac{\alpha \delta_{1}}{2(\tilde{\gamma}\sigma + 5D)}$. Therefore, we get
\begin{align}
\frac{1}{\beta^{2} L}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} \leq \frac{4 r(\tilde{\gamma \sigma} +5D)^{2} C_{1}}{n L}\left(\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\|^{2}\right)
\end{align}
and
\begin{align}
\|\hat{x}_{t+1} - \hat{x}_{t} \|^2 
&\leq  \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{100 \alpha^{2}}{n^{2}}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{4}+\frac{\left(M \alpha \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}\right]+\frac{6}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{\underline{u}}_{t} \right\|^{2} + \left\|\bar{\underline{u}}_{t}-\bar{u}_{t}\right\|^{2}\right) \nonumber\\
&\leq \frac{4}{\left(1-2 \delta_{1}^{2}\right)^{2}}\left[\frac{25 \alpha^{4} C_1 \delta_1^2}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left( \delta_{1} \beta\right)^{2}}{ n}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}\right]+\frac{6}{\left(1-2 \delta_{1}^{2}\right)^{2}} \beta^{2}\left(\left\|\bar{g}_{t}\right\|^{2}+\frac{1}{n}\left\|\mathbf{\underline{u}}_{t} \right\|^{2} + \left\|\bar{\underline{u}}_{t}-\bar{u}_{t}\right\|^{2}\right)  \nonumber
\end{align}
\begin{align}
\mathbb{E}\|\hat{x}_{t+1} - \hat{x}_{t} \|^2  \leq \frac{101 \alpha^{4} C_1 \delta_1^2}{n}\mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{ ( 5 \delta_{1}^2 + 7 )\beta^{2}}{ n}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{13}{2} \beta^{2}[\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{\tilde{\gamma}^2\sigma^2}{B}]
\end{align}

where we use $\alpha \leq \frac{1}{M}$ and $\frac{1}{\left(1-2 \delta_{1}^{2}\right)^{2}} \leq 1.002$. 

Therefore,
\begin{align}
&\mathbb{E}H_{t+1} - \mathbb{E}H_t \nonumber\\
\leq& 
\mathbb{E}\left\langle\bar{g}_{t}, \bar{x}_{t+1} - \bar{x}_t\right\rangle + \frac{\beta^{2} L}{2}\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\mathbb{E}\left\|\hat{x}_{t} - \bar{x}_{t}\right\|^{2} + \frac{1}{\beta^{2} L}\mathbb{E}\left\|\hat{x}_{t+1} - \bar{x}_{t+1}\right\|^{2} - L \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 - \frac{3 C_8 L^2}{n}\mathbb{E}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{18 L^2 \eta Q}{n}] \mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{18 L^2 \eta Q}{n}\mathbb{E}\|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \mathbb{E}\left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+  [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 18 L^2 \eta Q] \mathbb{E}\left\|\hat{x}_{t+1} - \hat{x}_{t}\right\|^{2} - [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 24 L^2 \eta^3 Q - 12 C_8 L^2 \eta^2]\mathbb{E}\left\|\bar{\underline{v}}_t\right\|^{2} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24 C_8 L^2}{Q}] \frac{Q}{n} \mathbb{E}\|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8 L^2 \eta^{2} - \frac{12 C_8 L^2 \eta}{Q} ] \frac{\eta Q}{n} \mathbb{E}\|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 \nonumber\\
\leq& - \beta\mathbb{E}\left\|\bar{g}_{t}\right\|^{2}+\frac{8 M D \alpha^{2}+2 D \alpha + L}{n}\mathbb{E}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} + \frac{\left(2 M D + L\right) \beta^{2}}{n}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + \frac{L}{2n}\mathbb{E}\left\|\mathbf{y}_{t} - \bar{\mathbf{y}}_{t}\right\|^{2} + \frac{\beta^{2} L}{2}\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} \nonumber\\
&- \frac{3 C_8 L^2}{n}\mathbb{E}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2+ \frac{100 r D^{2} C_{1}}{n L}\left(\mathbb{E}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2}+\mathbb{E}\left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\|^{2}\right) - L \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2  \nonumber\\
&+ [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n} + (1 + \frac{1}{c_0}) \frac{18L^2 \eta Q}{n}] \mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2}  + (1 + \frac{1}{c_0}) \frac{18L^2 \eta Q}{n} \mathbb{E}\|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  + [\frac{2 \eta L^2}{n} + \frac{67 L^3}{\mu^2 n}]  \mathbb{E}\left\|\mathbf{y}_{t}- \bar{\mathbf{y}}_{t}\right\|^{2} \nonumber \\
&+ [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 18L^2 \eta Q][\frac{101 \alpha^{4} C_1 \delta_1^2}{n}\mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{ ( 5 \delta_{1}^2 + 7 )\beta^{2}}{ n}\mathbb{E}\left\|\mathbf{u}_{t}\right\|^{2} + \frac{13}{2} \beta^{2}[\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{\tilde{\gamma}^2\sigma^2}{B}]]   \nonumber\\
&- [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 24 L^2 \eta^3 Q - 12 C_8 L^2  \eta^2]\left\|\bar{\underline{v}}_t\right\|^{2}  +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}  \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{24CL^2}{Q} ] \frac{Q}{n} \mathbb{E}\|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12 C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \mathbb{E}\|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 \nonumber\\
\leq& - [\beta - \frac{\beta^2 (L + 13C_2)}{2} ] \mathbb{E}\left\|\bar{g}_{t}\right\|^{2}  + \frac{\left(2 M D+L + C_2( 5 \delta_{1}^2 + 7)\right) \beta^{2}}{n}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} - \frac{3 C L^2}{n}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 \nonumber\\
&+ [\frac{100 r D^{2} C_{1}}{n L} + \frac{2 \eta L^2}{n} + \frac{67 \eta L^2}{3 \mu n} + (1 + \frac{1}{c_0}) \frac{6L^2 \eta Q}{n} + C_2\frac{101 \alpha^{4} C_1 \delta_1^2}{n} + \frac{8 M D \alpha^{2}+2 D \alpha + L}{n}] \mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} - L \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2  \nonumber\\
&+ [(1 + \frac{1}{c_0}) \frac{2L^2 \eta Q}{n} + \frac{100 r D^{2} C_{1}}{n L}] \mathbb{E}\|\mathbf{x}_{t+1} - \hat{\mathbf{x}}_{t+1} \|^2  \nonumber \\
&- [\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 24 L^2 \eta^3 Q - 12 C_8 L^2 \eta^2]\mathbb{E}\left\|\bar{v}_t\right\|^{2}  +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B} + \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B} \nonumber\\
&- [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{L}{2Q} -   [\frac{2 \eta L^2}{Q} + \frac{67 \eta L^2}{3 \mu Q}] - \frac{24C_8 L^2}{Q}] \frac{Q}{n} \mathbb{E}\|\mathbf{y}_t - \bar{\mathbf{y}}_t \|^2 \nonumber\\
&-[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12 C_8 L^2 \eta}{Q}] \frac{\eta Q}{n} \mathbb{E}\|\mathbf{\underline{v}}_t - \bar{\mathbf{\underline{v}}}_t \|^2 \nonumber\\
\end{align}
where we define $C_2 = [\frac{1}{2 \eta} + \frac{  L_{\Phi}}{2} + \frac{40 \kappa^{2}L}{ \mu^2 \eta^2 } + (1 + \frac{1}{c_0}) 18L^2 \eta Q]$ and we also need $[\frac{6 \eta L}{\mu} - (1 + \frac{1}{c_0}) 16 L^2 \eta^3 Q - 12 C_8 L^2 \eta^2] \geq 0, [1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0}) 16L^2 \eta - \frac{L}{2Q} -   [\frac{2 \eta L^2}{Q} + \frac{25 \eta L^2}{3 \mu Q}] - \frac{24C_8 L^2}{Q}] \geq 0$, and $[1 - (1 + c_0)\lambda^2 - (1 + \frac{1}{c_0})\eta - (1 + \frac{1}{c_0}) 8L^2 \eta^{2} - \frac{12 C_8 L^2 \eta}{Q}] \geq 0$, Let $c_0 = \frac{1}{\lambda} - 1, Q = 48 C_8 L^2$ and $\eta \leq \min \{\frac{1}{8 C_8 L^2}, \frac{1}{32L^2(1 + \frac{1}{c_0})} \}$

Recall that
% \begin{align}
% \left\|\mathbf{x}_{t+1}-\hat{\mathbf{x}}_{t+1}\right\| \leq \rho_{t}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\| + \beta\left\|\mathbf{\underline{u}}_{t}\right\| .
% \end{align}
% We apply the Lemma \ref{lem:13}
\begin{align} \label{eq:131}
\frac{1}{n} \sum_{t=0}^{T}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} \leq C_3 \frac{\beta^{2}}{n} \sum_{t=0}^{T}\left\|\mathbf{\underline{u}}_{t}\right\|^{2}
\end{align}

where $C_3 = \frac{2}{\left(1-\rho_{t}\right)^{2}}$.

Then we have
\begin{align} \label{eq:132}
& \mathbb{E}H_{T} - \mathbb{E}H_0 \nonumber\\
\leq& - [\beta - \frac{\beta^2 (L + 13C_2)}{2} ]\sum_{t=0}^{T-1} \mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{C_5}{n} \beta^2 \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|
+ \frac{C_6}{n} \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{C_7}{n} \sum_{t=1}^{T+1}\mathbb{E}\left\|\mathbf{x}_{t}-\hat{\mathbf{x}}_{t}\right\|^{2} - L \sum_{t=0}^{T-1} \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
&- \frac{3 C_8 L^2}{n}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbf{y}_{T} - \mathbf{y}_{t} \|^2\nonumber\\
\leq & - [\beta - \frac{\beta^2 (L + 13C_2)}{2} ]\sum_{t=0}^{T-1} \mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + (C_5 + C_6 C_3 + C_7 C_3)
\frac{\beta^{2}}{n} \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + C_4  - L \sum_{t=0}^{T-1} \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber \\
&- \frac{3 C L^2}{n}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B} + \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B} \nonumber\\
\end{align}

where we use $\beta \leq \min \{\frac{1}{L + 13 C_2 }, \frac{\alpha \delta_{1}}{2(\tilde{\gamma}\sigma + 5D)}\}, \beta^{2}\left\|\mathbf{u}_{T}\right\|^{2}  \leq \frac{\delta_{1}^{2} \alpha^{2} n}{4}$ and $C_4=\frac{C_3 C_7 \delta_{1}^{2} \alpha^{2}}{4} $ in the last inequality.
% We are going to associate $\left\|\bar{g}_{t}\right\|^{2}$ with $\left\|\mathbf{u}_{t}\right\|^{2}$. 
% We have the fact that 
% \begin{align}
% \left\|\mathbf{u}_{t}\right\| \leq\left\|\mathbf{u}_{t}-\bar{\mathbf{g}}_{t}\right\| + \left\|\bar{\mathbf{g}}_{t}\right\|
% \end{align}
Recall we have 
\begin{align}
-\sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2}= -\frac{1}{n} \sum_{t=0}^{T-1}\left\|\bar{\mathbf{g}}_{t}\right\|^{2} \leq \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\|^{2} - \frac{1}{2 n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2}
\end{align}
% and
% \begin{align}
% \left\|\mathbf{u}_{t+1} - \bar{\mathbf{g}}_{t+1}\right\| \leq \sigma_{2}^{t}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\| + \left\|\mathbf{g}_{t+1} - \mathbf{g}_{t}\right\|
% \end{align}
% we have 
\begin{align}
\frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t} - \bar{\mathbf{g}}_{t}\right\|^{2} &\leq C_8 \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{g}_{t+1} - \mathbf{g}_{T}\right\|^{2} \nonumber\\
&\leq C_8 \frac{1}{n} \sum_{t=0}^{T-1}\left(12 \alpha^{2} L^{2}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + 3 \beta^{2} L^{2}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + 3 L^2\|y_{t+1} - y_t\|^2\right) \nonumber\\
&\leq \left(12 \alpha^{2} C_3 C_8 + 3 C_8\right) L^{2} \beta^{2} \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + 3 C_8 L^2 \frac{1}{n} \sum_{t=0}^{T-1}\|y_{t+1} - y_t\|^2  
% &\leq\left(8 \tilde{C}_{0}+\frac{1}{2} \tilde{C}_{2}\right) \alpha \delta_{1} L \beta \frac{1}{n} \sum_{k=0}^{K}\left\|\mathbf{u}_{t}\right\|_{\mathrm{F}}^{2}+8 \alpha^{2} \tilde{C}_{1} \tilde{C}_{2} L^{2}+\tilde{C}_{3} + 3 C_8 L^2 \frac{1}{n} \sum_{t=0}^{T}\|y_{t+1} - y_t\|^2 
\end{align}
where  $C_8 = \frac{2}{\left(1-\sigma_{2}^{t}\right)^{2}}$. 
% The last line is due to $\beta \leq \frac{\alpha \delta_{1}}{5 L}$ and $\alpha^{2} \tilde{C}_{2} \leq \tilde{C}_{2} \leq$ $\frac{2}{\left(1-\frac{1}{2 \sqrt{n}}\right)^{2}} \leq 5$. 
\begin{align}
-\sum_{t=0}^{T-1}\left\|\bar{g}_{t}\right\|^{2} \leq \left[\left(24 \alpha^{2} C_3 C_8 + 6 C_8\right) L^{2} \beta^{2} - \frac{1}{2}\right] \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t}\right\|^{2} + (24 \alpha^{2} C_3 C_8 + 6 C_8) L^{2} \beta^{2} \frac{1}{n} \sum_{t=0}^{T-1}\left\|\mathbf{u}_{t} - \mathbf{\underline{u}}_{t}\right\|^{2} +  3L^2 C_8 \frac{1}{n} \sum_{t=0}^{T-1} \|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 
% +  12 \alpha^{2} C_4 C_8 L^{2} + C_9
\end{align}

Hence, following \eqref{eq:132}, we have
\begin{align}
& \mathbb{E}H_{T} - \mathbb{E}H_0 \nonumber\\
\leq & - \frac{\beta}{2}\sum_{t=0}^{T-1} \mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + (C_5 + C_6 C_3 + C_7 C_3)
\frac{\beta^{2}}{n} \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{\underline{u}}_{t}\right\|^{2} + C_4  - L \sum_{t=0}^{T-1}\mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber \\
&- \frac{3 C L^2}{n}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbf{y}_{t+1} - \mathbf{y}_{t} \|^2 +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}T + \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B}T \nonumber\\
\leq & - \frac{\beta}{2}[ \frac{1}{2} - \left(24 \alpha^{2} C_3 C_8 + 6 C_8\right) L^{2} \beta^{2} - 2(C_5 + C_6 C_3 + C_7 C_3)\beta]  
\frac{1}{n} \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{u}_{t}\right\|^{2} + C_{4} - L \sum_{t=0}^{T-1}\mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 \nonumber\\
+& [2(C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2] \frac{\beta^{2} \tilde{\gamma}\sigma}{B}T +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}T + \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B}T \nonumber\\
\leq & - \frac{\beta}{10n}  \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{u}_{t}\right\|^{2} + C_{4} - L \sum_{t=0}^{T-1} \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 + [2(C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta^{2} \tilde{\gamma}\sigma}{B}T \nonumber\\
&+  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}T + \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B}T 
\end{align}
where $ \beta \leq \beta_0 = \min \{\frac{1}{5\sqrt{(24 \alpha^{2} C_3 C_8 + 6 C_8)L^2}}, \frac{1}{10(C_5 + C_6 C_3 + C_7 C_3)} \}$

Then, we get
\begin{align}
\frac{\beta}{10} \sum_{t=0}^{T-1}\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} \leq \frac{\beta}{10} \cdot \frac{1}{n} \sum_{t=0}^{T-1}\mathbb{E}\left\|\mathbf{u}_{t}\right\|^{2} \leq& \mathbb{E}H_{0} - \mathbb{E}H_T + C_{4} - \sum_{t=0}^{T-1} L \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 +  6 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B}T \nonumber\\
&+ \frac{13C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{2B}T +  [2(C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta^{2} \tilde{\gamma}\sigma}{B}T \nonumber
\end{align}
\begin{align}
\frac{1}{T} \sum_{t=0}^{T-1}[\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{10L}{\beta} \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2]]\leq& 10\frac{\mathbb{E}H_{0} - \mathbb{E}H_T + C_{4}}{T \beta} +  60 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B \beta} + \frac{65 C_2 \beta \tilde{\gamma}^2\sigma^2}{B} \nonumber\\
&+ [2(C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta \tilde{\gamma}\sigma}{B}
\end{align}

Then with \eqref{eq:131}, we have
\begin{align}
\frac{1}{T} \sum_{i=0}^{T-1}[\frac{1}{n}\mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + 20\beta C_3 L \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \leq& \frac{20 \beta( H_0 - H_{T} + C_{4}) C_3 }{T} +  120 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B} + \frac{130 C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{B} \nonumber\\
&+ [2(C_3 + C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta^{2} \tilde{\gamma}\sigma}{B}
\end{align}

So,
\begin{align}
\frac{1}{T} \sum_{i=0}^{T-1} \mathbb{E}\mathfrak{M}_t &= \frac{1}{T} \sum_{i=0}^{T-1}[\mathbb{E}\left\|\bar{g}_{t}\right\|^{2} + \frac{1}{n}\mathbb{E}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{L}{n} \mathbb{E}\|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \nonumber\\
&\leq 
\frac{1}{T} \sum_{i=0}^{T-1}[ \left\|\bar{g}_{t}\right\|^{2} + \frac{10 L}{ \beta} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2 + \frac{1}{n}\left\|\mathbf{x}_{t} - \hat{\mathbf{x}}_{t}\right\|^{2} + \frac{20\beta C_3 L}{n} \|\bar{y}_t - y_t^{*}(\hat{x}_t) \|^2] \nonumber\\
&\leq 10\frac{\mathbb{E}H_{0} - \mathbb{E}H_T + C_{4}}{T \beta} + \frac{20 \beta( H_0 - H_{T} + C_{4}) C_3 }{T}\nonumber\\
&+ 60 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B \beta} + 120 \eta Q(1 + \frac{1}{c_0}) \frac{\sigma^2}{B} + \frac{65 C_2 \beta \tilde{\gamma}^2\sigma^2}{B} + \frac{130 C_2 \beta^2 \tilde{\gamma}^2\sigma^2}{B}\nonumber\\
&+ [2(C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta \tilde{\gamma}\sigma^2}{B}\nonumber\\ 
&+ [2(C_3 + C_5 + C_6 C_3 + C_7 C_3) + (24 \alpha^{2} C_3 C_8 + 6 C_8)L^2]  \frac{\beta^{2} \tilde{\gamma}\sigma^2}{B} \nonumber\\
&\leq 10\frac{\mathbb{E}H_{0} - \mathbb{E}H_T + C_{4}}{T \beta} + \frac{20 \beta( H_0 - H_{T} + C_{4}) C_3 }{T} + \frac{C_9 \sigma^2}{B}
\end{align}
\end{proof}


\section{Model Architectures in the Experiments}
The output number O for the orthonormal fair classification networks tasks is 3 while for the distributionally robust optimization is 10.
\vspace*{-6pt}
\begin{table*} [h]
  \centering
  \vspace*{-6pt}
  \caption{Model Architecture for MNIST }
  \label{tab:3}
    \vspace*{-6pt}
\begin{tabular}{ll}
\hline Layer Type & Shape \\
\hline Convolution + ReLU & $5 \times 5 \times 20 $ \\
Max Pooling & $2 \times 2$ \\
Convolution + ReLU & $5 \times 5 \times 50$ \\
Max Pooling & $2 \times 2$ \\
Fully Connected + ReLU & 500 \\
Fully Connected + ReLU & O \\
\hline
\end{tabular}
\vspace*{-6pt}
\end{table*}
\vspace*{-6pt}
\begin{table*} [th]
  \centering
 \vspace*{-6pt}
 \caption{ Model Architecture for Fashion-MNIST }
 \label{tab:4}
 \vspace*{-6pt}
\begin{tabular}{ll}
\hline Layer Type & Shape \\
\hline Convolution & $3 \times 3 \times 32 $ \\
Max Pooling & $2 \times 2$ \\
Convolution + ReLU & $3 \times 3 \times 64$ \\
Max Pooling & $2 \times 2$ \\
Fully Connected + ReLU & 128 \\
Fully Connected + ReLU & O \\
\hline
\end{tabular}
\end{table*}
\vspace*{-6pt}
\begin{table*} [th]
  \centering
    \vspace*{-6pt}
  \caption{ Model Architecture for CIFAR-10 }
  \label{tab:5}
    \vspace*{-6pt}
\begin{tabular}{llc}
\hline Layer Type & Shape \\
\hline Convolution + ReLU & $3 \times 3 \times 32 $ \\
Max Pooling & $2 \times 2$ \\
Convolution + ReLU & $3 \times 3 \times 64$  \\
Max Pooling & $2 \times 2$ \\
Convolution + ReLU & $3 \times 3 \times 64$  \\
Max Pooling & $2 \times 2$ \\
Fully Connected + ReLU & 200 \\
Fully Connected + ReLU & O \\
\hline
\end{tabular}
\end{table*}
